Precision and Sensitivity in Detailed-Balance Reaction Networks

We study two specific measures of quality of chemical reaction networks, Precision and Sensitivity. The two measures arise in the study of sensory adaptation, in which the reaction network is viewed as an input-output system. Given a step change in input, Sensitivity is a measure of the magnitude of the response, while Precision is a measure of the degree to which the system returns to its original output for large time. High values of both are necessary for high-quality adaptation. We focus on reaction networks without dissipation, which we interpret as detailed-balance, mass-action networks. We give various upper and lower bounds on the optimal values of Sensitivity and Precision, characterized in terms of the stoichiometry, by using a combination of ideas from matroid theory and differential-equation theory. Among other results, we show that this class of non-dissipative systems contains networks with arbitrarily high values of both Sensitivity and Precision. This good performance does come at a cost, however, since certain ratios of concentrations need to be large, the network has to be extensive, or the network should show strongly different time scales.

==> chemfig.tex <==
%  __________________________________________________________________
% |                                                                  |
% |                                                                  |
% |                           chemfig v1.1a                          |
% |                                                                  |
% |                         23 february 2015                         |
% |                                                                  |
% |__________________________________________________________________|
%
% This is chemfig.tex, the code of the "chemfig" package.
%
% Maintainer: Christian Tellechea
% E-mail    : unbonpetit@openmailbox.org
%             Comments, bug reports and suggestions are welcome.
% Licence   : Released under the LaTeX Project Public License v1.3c or
%             later, see http://www.latex-project.org/lppl.txt
% Copyright : Christian Tellechea 2010-2015
%
% The "chemfig" package consists of the 8 following files:
%    - chemfig.tex (this file)
%    - chemfig.sty (the package file for LaTeX)
%    - t-chemfig.tex (the package file for conTeXt)
%    - README
%    - chemfig_doc_en.tex, chemfig_doc_en.pdf (english manual)
%    - chemfig_doc_fr.tex, chemfig_doc_fr.pdf (manual in french)
%
% --------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
% %     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% --------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% --------------------------------------------------------------------

\def\usechemfigcatcode{%
	\begingroup
		\def\X##1{\catcode\number`##1=\number\catcode`##1\relax}
		\xdef\chemfigrestorecatcode{%
			\X\[\X\]\X\:\X\(\X\)\X\,\X\-\X\=\X\~\X\!\X\?\X\<\X\>\X\;\X\*\X\|\X\@\X\
			\let\noexpand\chemfigrestorecatcode\relax
		}%
	\endgroup
	\catcode`\[12 \catcode`\]12 \catcode`\:12 \catcode`\(12
	\catcode`\)12 \catcode`\,12 \catcode`\-12 \catcode`\=12
	\catcode`\~12 \catcode`\!12 \catcode`\?12 \catcode`\<12
	\catcode`\>12 \catcode`\;12 \catcode`\*12 \catcode`\|12
	\catcode`\@11 \catcode`\#6  \catcode`\ 10
}

\usechemfigcatcode

% V\'erifie que eTeX est le moteur utilis\'e
\begingroup
	\edef\CF@ver{\meaning\eTeXversion}
	\edef\CF@date{\string\eTeXversion}
	\ifx\CF@ver\CF@date
		\endgroup
	\else
		\endgroup
		\errmessage{Package chemfig Error: you are not using the eTeX engine, chemfig cannot work and is not loaded.}%
		\expandafter\endinput
	\fi

\def\CF@def#1{%
	\ifdefined#1%
		\errmessage{Package chemfig Error: the macro \string#1\space is already defined. Please, email the author.}%
	\fi
	\def#1%
}

\CF@def\CF@ver         {1.1a}
\CF@def\CF@date        {2015/02/23}
\CF@def\CF@fr@date     {23 f\'evrier 2015}
\CF@def\CF@en@date     {23 february 2015}
\CF@def\CF@package@name{chemfig}

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\ifdefined\tikzpicture\else
		\def\CF@next@action{\input tikz.tex}%
		\expandafter\CF@next@action
	\fi
	\immediate\write\m@ne{Package: \CF@package@name\space\CF@date\space\space v\CF@ver\space\space Draw molecule with an easy syntax}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@firstofone#1{#1}
	\long\def\@gobble#1{}
	\long\def\@gobbletwo#1#2{}
	\def\@car#1#2\@nil{#1}
	\def\@makeother#1{\catcode`#1=12\relax}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
	\def\space{ }
	\CF@def\printatom#1{\ifmmode\rm#1\else$\rm#1$\fi}% \printatom pour TeX et ConTeXt
\else% fin des d\'efinitions LaTeX
	\CF@def\printatom#1{\ensuremath{\mathrm{#1}}}% \printatom pour LaTeX.
\fi

\CF@def\CF@ifx#1#2{\ifx#1#2\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi}

\newcount\CF@cnt@atomingroup
\newcount\CF@cnt@groupnumber
\newcount\CF@cnt@atomnumber
\newcount\CF@cnt@cycle

\newif\ifCF@incycle
\newif\ifCF@cyclearc
\newif\ifCF@definesubmol
\newif\ifCF@name@dp@adjust
\newif\ifCF@macrofixedbondlength
\newif\ifCF@globalfixedbondlength
\def\enablefixedbondlength{\global\CF@globalfixedbondlengthtrue}
\def\disablefixedbondlength{\global\CF@globalfixedbondlengthfalse}
\disablefixedbondlength

\newdimen\CF@dim

\newbox\CF@lewis@box
\newbox\CF@box@boxa
\newbox\CF@box@boxb
\newbox\CF@stuff@box

\newwrite\CF@unused

\CF@def\CF@sanitize@catcode{%
	\@makeother\[\@makeother\]\@makeother\:\@makeother\(\@makeother\)%
	\@makeother\,\@makeother\-\@makeother\=\@makeother\~\@makeother\!%
	\@makeother\?\@makeother\<\@makeother\>\@makeother\;\@makeother\*%
	\@makeother\|\@makeother\#\@makeother\@%
}

\CF@def\CF@node@content{\expandafter\printatom\expandafter{\csname atom@\number\CF@cnt@atomnumber\endcsname\CF@node@strut}}

\CF@def\chemskipalign{%
	\ifx\CF@bond@outcontentsaved\@empty% sauf si un \chemskipalign a \'et\'e fait \`a l'atome pr\'ec\'edent
		\global\let\CF@bond@outcontentsaved\CF@bond@outcontent% sauvegarder l'atome d'o\`u vient la liaison
	\fi
	\let\CF@node@strut\@empty
}

\CF@def\CF@empty@node{{}}

\CF@def\CF@cycle@inraduiscoeff{0.75}% coeff multiplicateur du rayon des arcs dans les cycles

\CF@def\setcrambond#1#2#3{%
	\def\CF@cram@basewidth{#1}%
	\ifx\@empty#2\@empty\def\CF@cram@dashlength{1pt}\else\def\CF@cram@dashlength{#2}\fi
	\ifx\@empty#3\@empty\def\CF@cram@dashsep{2pt}\else\def\CF@cram@dashsep{#3}\fi}
\setcrambond{}{}{}

\CF@def\setatomsep{\def\CF@atom@sep}% espacement des atomes li\'es
\setatomsep{}

\CF@def\setbondoffset{\def\CF@bond@offset}% offset des liaisons
\setbondoffset{2pt}

\CF@def\setdoublesep{\def\CF@double@sep}
\setdoublesep{2pt}

\CF@def\definesubmol{\CF@definesubmoltrue\CF@def@submol}
\CF@def\redefinesubmol{\CF@definesubmolfalse\CF@def@submol}

\CF@def\CF@def@submol#1{%
	\begingroup
		\def\CF@tmp@str{#1}%
		\catcode`[\@ne\catcode`]\tw@
		\futurelet\CF@toks@a\CF@test@nxttok
}

\CF@def\CF@test@nxttok{%
	\if[\noexpand\CF@toks@a\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\expandafter\CF@grab@optalias\expandafter{\CF@tmp@str}}%
		{\CF@expand@second{%
			\endgroup
			\begingroup
			\CF@sanitize@catcode
			\CF@def@submol@i
			}\CF@tmp@str{}%
		}%
}

\CF@def\CF@grab@optalias#1#2{%
	\endgroup
	\begingroup
	\everyeof{\@nil}\endlinechar\m@ne
	\CF@sanitize@catcode
	\expandafter\assign@tonil\expandafter\CF@tmp@str\scantokens{#2}%
	\CF@expand@second{%
		\CF@sanitize@catcode
		\CF@def@submol@i{#1}%
		}\CF@tmp@str
}

\CF@def\CF@def@submol@i#1#2#3{% #1 nom, #2 = code si liaison arrive de droite , #3 = code si liaison arrive de gauche
	\endgroup
	\ifcat\relax\expandafter\noexpand\@car#1\@nil% si #1 est une s\'equence de contr\^ole
		\expandafter\ifdefined\@car#1\@nil
			\ifCF@definesubmol
				\immediate\write\CF@unused{Package \CF@package@name\space Warning: the macro \expandafter\string\@car#1\@nil\space is already defined, the previous definition is lost on input line \the\inputlineno.}%
			\fi
		\fi
		\ifx\@empty#2\@empty
			\CF@expand@second{\expandafter\def\@car#1\@nil}{\expandafter\@empty\romannumeral-`\.\noexpand#3}%
		\else
			\expandafter\def\@car#1\@nil{%
				\romannumeral-`\.% donnera le d\'eveloppement souhait\'e en 1 coup
				\ifdim\CF@current@angle pt>90pt
					\ifdim\CF@current@angle pt<270pt
						\expandafter\expandafter\expandafter\@firstoftwo
					\else
						\expandafter\expandafter\expandafter\@secondoftwo
					\fi
				\else
					\expandafter\@secondoftwo
				\fi
				{\noexpand#2}{\noexpand#3}}%
		\fi
	\else
		\ifcsname CF@@#1\endcsname
			\ifCF@definesubmol
				\immediate\write\CF@unused{Package \CF@package@name\space Warning:the submol "#1" is already defined, the previous definition is lost on input line \the\inputlineno.}%
			\fi
		\fi
		\ifx\@empty#2\@empty
			\CF@expand@second{\expandafter\def\csname CF@@#1\endcsname}{\expandafter\@empty\romannumeral-`\.\noexpand#3}%
		\else
			\expandafter\def\csname CF@@#1\endcsname{%
				\romannumeral-`\.% donnera le d\'eveloppement souhait\'e en 1 coup
				\ifdim\CF@current@angle pt>90pt
					\ifdim\CF@current@angle pt<270pt
						\expandafter\expandafter\expandafter\@firstoftwo
					\else
						\expandafter\expandafter\expandafter\@secondoftwo
					\fi
				\else
					\expandafter\@secondoftwo
				\fi
				{\noexpand#2}{\noexpand#3}}%
		\fi
	\fi
}

\CF@def\CF@if@integer#1{%
	\begingroup
		\afterassignment\CF@after@integer
		\CF@cnt@cycle0#1\relax
}

\CF@def\CF@after@integer#1\relax{%
	\endgroup
	\CF@ifx{\@empty#1}\@empty
}

\CF@def\CF@swap@fi#1\fi{\fi#1}

\CF@def\CF@gobble@tonil#1\@nil{}

\CF@def\CF@expafterarg@ntimes#1#2#3{%
	\CF@expafterarg@ntimes@i{#1}{#3}%
	\expandafter\CF@swap@arg\expandafter{\CF@tmp@str}{#2}%
}

\CF@def\CF@expafterarg@ntimes@i#1#2{%
	\ifnum#1=\z@
		\def\CF@tmp@str{#2}%
	\else
		\CF@swap@fi
		\expandafter\CF@expafterarg@ntimes@i\expandafter{\number\numexpr#1-1\expandafter}\expandafter{#2}%
	\fi
}

\CF@def\CF@swap@arg#1#2{#2{#1}}

\CF@def\CF@expand@second#1#2{\expandafter\CF@swap@arg\expandafter{#2}{#1}}

\CF@def\CF@swap@char#1#2{#2#1}

\CF@def\CF@expand@afterfirst#1#2{\expandafter\CF@swap@char\expandafter{#2}{#1}}

\CF@def\CF@edef@second#1#2{%
	\edef\CF@tmp@str{#2}%
	\expandafter\CF@swap@char\expandafter{\CF@tmp@str}{#1}%
}

\CF@def\CF@add@tocs#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\CF@def\CF@expadd@tocs#1#2{\expandafter\CF@add@tocs\expandafter#1\expandafter{#2}}

\CF@def\CF@edefadd@tocs#1#2{%
	\edef\CF@tmp@str{#2}%
	\expandafter\CF@add@tocs\expandafter#1\expandafter{\CF@tmp@str}%
}

\CF@def\CF@if@firsttokmatch#1#2{% est ce que #1 et #2 commencent par les m\^emes tokens ?
	\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
	\futurelet\CF@toks@b\CF@gobble@tonil#2\relax\@nil
	\CF@ifx\CF@toks@a\CF@toks@b
}

\CF@def\CF@if@firsttokin#1{% teste si le token qui commence #1 appartient aux tokens mis dans #2
	\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
	\CF@if@firsttokin@i
}

\CF@def\CF@if@firsttokin@i#1{%
	\ifx\@empty#1\@empty
		\expandafter\@secondoftwo
	\else
		\futurelet\CF@toks@b\CF@gobble@tonil#1\relax\@nil
		\ifx\CF@toks@a\CF@toks@b
			\expandafter\expandafter\expandafter\@firstoftwo
		\else
			\CF@swap@fi\CF@swap@fi
			\expandafter\CF@if@firsttokin@i\expandafter{\@gobble#1}%
		\fi
	\fi
}

\CF@def\CF@if@instr#1#2{%
	\def\CF@if@instr@i##1#2##2\@nil{\ifx\@empty##2\@empty\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}%
	\CF@if@instr@i#1\@@nil#2\@nil
}

\CF@def\CF@after@space#1 #2\@nil{#2}

\CF@def\CF@seek@node#1#2#3{% cherche un noeud au d\'ebut de #1 l'assigne dans la sc #2 et met le reste dans #3
	\let#2\@empty
	\def#3{#1}%
	\CF@if@firsttokmatch{#1}{ }%
		{\expandafter\CF@seek@node@i\expandafter{\romannumeral-`\.\noexpand#1}#2#3}% ignore les espaces au d\'ebut du groupe d'atome
		{\CF@seek@node@i{#1}#2#3}%
}

\CF@def\CF@seek@node@i#1#2#3{%
	\ifx\@empty#1\@empty
		\let#3\@empty
	\else
		\futurelet\CF@toks@a\CF@gobble@tonil#1\relax\@nil
		\CF@ifx\CF@toks@a\@sptoken
			{\CF@add@tocs#2{ }%
			\CF@swap@fi\expandafter\CF@seek@node@i\expandafter{\CF@after@space#1\@nil}#2#3%
			}%
			{\CF@ifx\CF@toks@a\bgroup
				{\CF@expadd@tocs#2{\expandafter{\@car#1\@nil}}%
				\CF@swap@fi\expandafter\CF@seek@node@i\expandafter{\@gobble#1}#2#3%
				}%
				{\CF@if@firsttokin@i{-=(*<>!~}%
					{\def#3{#1}}%
					{\CF@expadd@tocs#2{\@car#1\@nil}%
					\CF@swap@fi\expandafter\CF@seek@node@i\expandafter{\@gobble#1}#2#3%
					}%
				}%
			}%
	\fi
}

% on sait que #1 commence par -,=,~,<,>. On analyse cette liaison
% #2 reçoit le type de liaisons (1 pour -, 2 pour =, 3 pour ~)
\CF@def\CF@bond@findcode#1#2{%
	\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
	\edef#2{%
		\ifx-\CF@toks@a1%
		\else
			\ifx=\CF@toks@a2%
			\else
				\ifx~\CF@toks@a3%
				\else
					\ifx>\CF@toks@a4%
					\else
						\ifx<\CF@toks@a5%
						\else0% si 0 --> il y a une erreur non due \`a l'utilisateur
						\fi
					\fi
				\fi
			\fi
		\fi}%
	\ifnum#2>\thr@@% si c'est une liaison de Cram
		\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\@gobble#1\@nil% chope le caract\`ere suivant
		\ifx:\CF@toks@a
			\edef#2{\number\numexpr#2+2}% si c 'est un ":", signe du pointill\'e, ajoute 2
		\else
			\ifx|\CF@toks@a
				\edef#2{\number\numexpr#2+4}% si c 'est un "|", signe du triangle \'evid\'e, ajouter 4
			\fi
		\fi
	\fi
}

\CF@def\CF@analyse@bondoffset#1,#2\@nil{%
	\def\CF@start@offset{#1}\def\CF@end@offset{#2}%
}

\CF@def\CF@grab@bondoffset#1(#2)#3\@nil{%
	\ifx\@empty#2\@empty
	\else
		\CF@if@instr{#2},%
			{\CF@analyse@bondoffset#2\@nil}%
			{\def\CF@start@offset{#2}}%
	\fi
	\def\CF@remain@afterbond{#3}%
}

\CF@def\CF@analyse@bond#1#2{%
	\CF@bond@findcode{#1}#2%
	\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobble#1}%mange le premier signe de la liaison
	\let\CF@doublebond@type\z@
	\ifnum#2=\tw@% si c'est une double liaison, regarde s'il y a un + ou - derri\`ere
		\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\@gobble#1\@nil
		\ifx^\CF@toks@a
			\let\CF@doublebond@type\@ne
			\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobbletwo#1}% mange le "^"
		\else
			\ifx_\CF@toks@a
				\let\CF@doublebond@type\tw@
				\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobbletwo#1}% mange le "_"
			\fi
		\fi
	\else
		\ifnum#2>5 % si c'est une laision de Cram pointill\'ee ou triangle \'evid\'e
			\expandafter\def\expandafter\CF@remain@afterbond\expandafter{\@gobbletwo#1}% mange un caract\`ere de plus
		\fi
	\fi
	\expandafter\expandafter\expandafter\CF@if@firsttokmatch\expandafter\expandafter\expandafter{\expandafter\CF@remain@afterbond\expandafter}\string##%
		{\expandafter\CF@grab@bondoffset\CF@remain@afterbond\@nil}%
		\relax
	\expandafter\expandafter\expandafter\CF@if@firsttokmatch\expandafter\expandafter\expandafter{\expandafter\CF@remain@afterbond\expandafter}\string @%
		{\expandafter\CF@grab@movearg\CF@remain@afterbond\@nil}%
		\relax
	\expandafter\CF@if@firsttokmatch\expandafter{\CF@remain@afterbond}[%
		{\expandafter\CF@analyse@optarg\CF@remain@afterbond\@nil\CF@remain@afterbond}%
		{\let\CF@current@stringangle\CF@default@stringangle
		\let\CF@current@length\CF@default@length
		\let\CF@current@fromatom\CF@default@fromatom
		\let\CF@current@toatom\CF@default@toatom
		\let\CF@current@tikz\CF@default@tikz
		\let\CF@movebond@name\@empty
		}%
	\ifCF@incycle
		\pgfmathparse{360/\CF@cycle@num+\CF@initcycle@angle}%
		\let\CF@cycle@increment@angle\pgfmathresult
		\edef\CF@current@stringangle{::+\pgfmathresult}%
		\def\CF@initcycle@angle{0}%
		\let\CF@current@length\CF@default@length% et on ignore la longueur de liaison sp\'ecifi\'ee
	\fi
	\expandafter\CF@set@bondangle\expandafter{\CF@current@stringangle}\CF@current@angle
}

\CF@def\CF@set@bondangle#1#2{% le code de la direction est contenu dans #1, en sortie, #2 contient l'angle
	\ifx\@empty#1\@empty%
		\let#2\CF@default@angle
	\else
		\if:\expandafter\noexpand\@car#1\@nil
			\if:\expandafter\expandafter\expandafter\noexpand\expandafter\@car\@gobble#1\@nil
				\pgfmathparse{\CF@previous@angle+\expandafter\@gobble\@gobble#1}%
				\let#2\pgfmathresult
			\else
				\expandafter\def\expandafter#2\expandafter{\@gobble#1}%
			\fi% puis normalise l'angle entre 0 et 360
			\ifdim\ifdim#2pt<\z@-\fi#2pt>360pt % si |#2|>360
				\pgfmathparse{#2-360*floor(#2/360)}%
				\ifdim\pgfmathresult pt<\z@\pgfmathparse{\pgfmathresult+360}\fi
				\let#2\pgfmathresult
			\else
				\ifdim#2pt<\z@
					\pgfmathparse{#2+360}%
					\let#2\pgfmathresult
				\fi
			\fi
		\else
			\ifnum#1>7
				\pgfmathparse{#1-floor(#1/8)*8}%
				\ifdim\pgfmathresult pt<\z@\pgfmathparse{\pgfmathresult+8}\fi
				\edef#2{\ifcase\expandafter\CF@int@part\pgfmathresult\@nil0\or45\or90\or135\or180\or225\or270\or315\else-1\fi}% angle =-1 --> erreur
			\else
				\edef#2{\ifcase#1 0\or45\or90\or135\or180\or225\or270\or315\else-1\fi}%
			\fi
		\fi
	\fi
}

\CF@def\CF@int@part#1.#2\@nil{#1 }

\CF@def\CF@analyse@movearg#1,#2\@nil#3{%
	\def#3{#1}\def\CF@movebond@coeff{#2}%
}

% Argument limit\'es l\'egitimes ici car #2 (qui est ce qui suit "@{<nom>}" dans l'argument optionnel) ne DOIT
% pas commencer par une accolade.
\expandafter\CF@def\expandafter\CF@grab@movearg\string @#1#2\@nil{%
	\CF@if@instr{#1},%
		{\CF@analyse@movearg#1\@nil\CF@movebond@name}%
		{\def\CF@movebond@name{#1}\def\CF@movebond@coeff{0.5}}%
	\def\CF@remain@optarg{#2}%
}

\CF@def\CF@testempty@andassign#1#2#3{\ifx\@empty#2\@empty\let#1#3\else\def#1{#2}\fi}

\CF@def\CF@sanitize@lastitem#1,\@empty#2\@nil{#1}

\CF@def\CF@parse@optlist#1,#2,#3,#4,#5\@nil{%
	\CF@testempty@andassign\CF@current@stringangle{#1}\CF@default@stringangle
	\CF@testempty@andassign\CF@current@length{#2}\CF@default@length
	\CF@testempty@andassign\CF@current@fromatom{#3}\CF@default@fromatom
	\CF@testempty@andassign\CF@current@toatom{#4}\CF@default@toatom
	\expandafter\CF@testempty@andassign\expandafter\CF@current@tikz\expandafter{\CF@sanitize@lastitem#5,\@empty\@nil}\CF@default@tikz
}%

\CF@def\CF@analyse@optarg[#1]#2\@nil#3{%
	\ifx\@empty#1\@empty
	\else
		\CF@expand@afterfirst{\CF@if@firsttokmatch{#1}}{\string @}%
			{\CF@grab@movearg#1\@nil}%
			{\let\CF@movebond@name\@empty
			\def\CF@remain@optarg{#1}}%
		\expandafter\CF@parse@optlist\CF@remain@optarg,\@empty,\@empty,\@empty,\@empty\@nil
		\def#3{#2}%
	\fi
}

\CF@def\CF@seek@submol{%
	\expandafter\def\expandafter\CF@remain@molecule\expandafter{\romannumeral-`\.\expandafter\noexpand\CF@remain@molecule}%
	\expandafter\CF@if@firsttokmatch\expandafter{\CF@remain@molecule}!%
		{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter
			\CF@remain@molecule\expandafter\expandafter\expandafter{\expandafter\@gobble\CF@remain@molecule}% enl\`eve le ``!''
		\ifcat\relax\expandafter\expandafter\expandafter\noexpand\expandafter\@car\CF@remain@molecule\@nil
			\CF@expafterarg@ntimes5{\def\CF@insert@submol}{\expandafter\@car\CF@remain@molecule\@nil}%
		\else
			\CF@expafterarg@ntimes3{\def\CF@insert@submol}{\csname CF@@\expandafter\@car\CF@remain@molecule\@nil\endcsname}%
		\fi
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\CF@remain@molecule\expandafter\expandafter\expandafter
			{\csname CF@insert@submol\expandafter\expandafter\expandafter\endcsname\csname @gobble\expandafter\endcsname\CF@remain@molecule}%
		\CF@seek@submol
		}%
		\relax
}

\CF@def\CF@insert@emptygroup#1{% ins\`ere {} au d\'ebut de la sc #1
	\expandafter\def\expandafter#1\expandafter{\expandafter{\expandafter}#1}%
}

\CF@def\chemfig{\@ifstar{\CF@macrofixedbondlengthtrue\chemfig@i}{\CF@macrofixedbondlengthfalse\chemfig@i}}

\CF@def\chemfig@i{\ifCF@globalfixedbondlength\CF@macrofixedbondlengthtrue\fi\@testopt\CF@chemfig@ii{}}

\CF@def\CF@chemfig@ii[#1]{\@testopt{\CF@chemfig@iii[#1]}{}}

\CF@def\CF@chemfig@iii[#1][#2]{%
	\edef\CF@tmp@str{[remember picture,every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@\ifx\@empty#2\@empty\else,#2\fi},baseline\ifx\@empty#1\@empty\else,#1\fi]}%
	\expandafter\tikzpicture\CF@tmp@str
	\begingroup
		\let\CF@hook@list\@empty
		\ifx\CF@atom@sep\@empty\def\CF@atom@sep{3em}\fi
		\ifx\CF@cram@basewidth\@empty\def\CF@cram@basewidth{1.5ex}\fi
		\CF@incyclefalse
		\CF@cnt@groupnumber\z@
		\let\CF@last@action\z@% 0=d\'ebut du dessin 1=trac\'e d'un noeud 2=trac\'e d'une liaison
		\let\CF@start@offset\@empty
		\let\CF@end@offset\@empty
		\let\CF@bond@outcontentsaved\@empty
		\def\CF@cycle@anglecorrection{180/\CF@cycle@num}%
		\def\CF@default@angle{0}%
		\def\CF@default@stringangle{:0}% angle pris par d\'efaut si le champ est vide
		\def\CF@default@length{1}%
		\let\CF@default@fromatom\@empty% numero de l'atome d'o\`u partent les liaisons par d\'efaut
		\let\CF@default@toatom\@empty% num\'ero de l'atome o\`u arrivent les laisons par d\'efaut
		\let\CF@default@tikz\@empty
		\let\CF@previous@bondangle\empty
		\let\CF@joinbond\z@
		\let\CF@previous@tikz\empty
		\everyeof{\@nil}\endlinechar\m@ne
		\CF@sanitize@catcode
		\CF@chemfig@iv
}

\CF@def\CF@chemfig@iv#1{%
	\expandafter\assign@tonil\expandafter\CF@remain@molecule\scantokens{#1}%
	\expandafter\CF@chemfig@v\expandafter{\CF@remain@molecule}%
	\endtikzpicture
	\let\CF@split@state\z@
}

\CF@def\CF@chemfig@v#1{% #1 est le code de la mol\'ecule
	\ifnum\CF@last@action=\thr@@
		\ifCF@incycle
			\def\CF@default@angle{0}%
		\else
			\ifnum\CF@cnt@cycle=\z@% si c'est le d\'ebut d'un cycle
				\pgfmathparse{\CF@previous@angle+180+\CF@cycle@anglecorrection}% on met la liaison \`a +180° + correction
			\else
				\pgfmathparse{\CF@previous@angle-90+180/\CF@cycle@num}% sinon \`a la bissectrice du sommet du cycle
			\fi
			\let\CF@default@angle\pgfmathresult
		\fi
		\let\CF@default@stringangle\@empty
	\fi
	\let\CF@current@angle\CF@default@angle
	\def\CF@remain@molecule{#1}%
	\CF@seek@submol% alias en premier ?
	\if[\expandafter\expandafter\expandafter\noexpand\expandafter\@car\CF@remain@molecule\@nil
		\expandafter\CF@analyse@optarg\CF@remain@molecule\@nil\CF@remain@molecule
		\expandafter\CF@set@bondangle\expandafter{\CF@current@stringangle}\CF@current@angle
		\let\CF@default@angle\CF@current@angle
		\let\CF@previous@angle\CF@current@angle
		\unless\ifx\@empty\CF@current@stringangle\let\CF@default@angle\CF@current@angle\fi
		\unless\ifx\@empty\CF@current@length\let\CF@default@length\CF@current@length\fi
		\unless\ifx\@empty\CF@current@fromatom\let\CF@default@fromatom\CF@current@fromatom\fi
		\unless\ifx\@empty\CF@current@toatom\let\CF@default@toatom\CF@current@toatom\fi
		\unless\ifx\@empty\CF@current@tikz\let\CF@default@tikz\CF@current@tikz\fi
		\CF@seek@submol
	\fi
	\edef\CF@default@stringangle{:\CF@default@angle}%
	\let\CF@current@length\CF@default@length
	\let\CF@current@fromatom\CF@default@fromatom
	\let\CF@current@toatom\CF@default@toatom
	\let\CF@current@tikz\CF@default@tikz
	\ifCF@incycle% si on commence un cycle
		\let\CF@current@angle\CF@previous@angle
		\ifCF@cyclearc% on doit tracer l'arc de cercle dans le cycle ?
			\pgfmathparse{\CF@cycle@inraduiscoeff*\CF@current@length*\CF@atom@sep/(2*tan(180/\CF@cycle@num))}%
			\let\CF@cyclearc@radius\pgfmathresult
			\pgfmathparse{\CF@current@angle+\CF@initcycle@angle+180/\CF@cycle@num+90}
			\let\CF@cyclearc@initangle\pgfmathresult
			\pgfmathparse{\CF@current@length*\CF@atom@sep/(2*sin(180/\CF@cycle@num))}%
			\node[at=(\CF@bond@outnode),shift=(\CF@cyclearc@initangle:\pgfmathresult pt)](arccenter){};% le centre de l'arc
			\node[at=(arccenter),shift=(\CF@cyclearc@startangle:\CF@cyclearc@radius pt)](initarc){};% le d\'ebut de l'arc
			\expandafter\draw\expandafter[\CF@cyclearc@directtikz](initarc) arc (\CF@cyclearc@startangle:\CF@cyclearc@endangle:\CF@cyclearc@radius pt);
		\fi
	\else
		\let\CF@current@angle\CF@default@angle
	\fi
	\ifnum\CF@last@action=\z@
		\let\CF@previous@angle\CF@default@angle
		\node(CF@node){};
		\expandafter\CF@if@firsttokin\expandafter{\CF@remain@molecule}{-=(*~?<>}%
			{\CF@insert@emptygroup\CF@remain@molecule}%
			\relax
	\fi
	\CF@chemfig@vi
}

\CF@def\CF@chemfig@vi{%
	\let\CF@next@action\CF@chemfig@vi% \`a priori, on reboucle
	\ifx\CF@remain@molecule\@empty
		\let\CF@next@action\endgroup
	\else
		\CF@seek@submol
		\expandafter\CF@seek@node\expandafter{\CF@remain@molecule}\CF@current@atomgroup\CF@remain@molecule
		\ifx\@empty\CF@current@atomgroup% pas de noeud pour commencer ?
			\def\CF@bond@outnode{n\CF@last@groupnumber-%
				 \ifx\CF@current@fromatom\@empty
					 \ifdim\CF@current@angle pt<90pt \number\CF@cnt@atomingroup
					 \else\ifdim\CF@current@angle pt>270pt \number\CF@cnt@atomingroup\else1\fi
					 \fi
				 \else\CF@current@fromatom
				 \fi}%
			\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\CF@remain@molecule\relax\@nil
			\CF@if@firsttokin@i{-=<>~}% la suite est une liaison
				{\ifnum\CF@last@action=\tw@% c'est la deuxi\`eme liaison cons\'ecutive ?
					\CF@insert@emptygroup\CF@remain@molecule% ins\`ere un groupe vide
					\edef\CF@bond@outnode{\CF@bond@outnode}%
				\else
					\ifCF@incycle\advance\CF@cnt@cycle\@ne\fi
					\expandafter\CF@analyse@bond\expandafter{\CF@remain@molecule}\CF@bond@type
					\edef\CF@bond@outnode{\CF@bond@outnode}%
					\let\CF@remain@molecule\CF@remain@afterbond
					\ifCF@incycle
						\ifnum\CF@cnt@cycle=\CF@cycle@num\relax
							\expandafter\expandafter\expandafter\@firstoftwo
						\else
							\ifnum\CF@cnt@cycle=\@ne
								\let\CF@cycle@firsttikz\CF@current@tikz
								\unless\ifx\CF@start@offset\@empty\let\CF@cycle@joinlast\z@\fi
							\fi
							\expandafter\expandafter\expandafter\@secondoftwo
						\fi
					\else
						\expandafter\@secondoftwo
					\fi
						{\let\CF@next@action\endgroup
						\CF@draw@bond\CF@bond@type{\CF@bond@outnode}{\CF@hook@cycle}\CF@previous@atomgroup\CF@hook@atomgroup
						}%
						{\node[at=(\CF@bond@outnode\ifCF@incycle\else\ifCF@macrofixedbondlength.\CF@current@angle\fi\fi),shift=(\ifcase\CF@split@state\or180-\or-\fi\CF@current@angle:\CF@current@length*\CF@atom@sep)](CF@node){};
						\let\CF@previous@angle\CF@current@angle
						\let\CF@last@action\tw@
						}%
				\fi
				\ifcat\relax\detokenize\expandafter{\romannumeral-`\.\expandafter\noexpand\CF@remain@molecule}\relax
				% s'il ne reste plus rien apr\`es la liaison (sans tenir compte de l'espace devant)-> ins\`ere un groupe vide
					\CF@insert@emptygroup\CF@remain@molecule
				\fi
				}%
				{\edef\CF@bond@outnode{\CF@bond@outnode}% \'evalue le l'atome de d\'epart de liaison
				\CF@ifx(\CF@toks@a% une parenth\`ese pour commencer ?
					{\ifnum\CF@last@action=\tw@% il y avait une liaison juste avant ?
						\CF@insert@emptygroup\CF@remain@molecule
					\else
						\expandafter\CF@grab@submol\expandafter{\CF@remain@molecule}%
						\begingroup
							\ifCF@incycle\let\CF@last@action\thr@@\fi% on \'etait dans un cycle
							\CF@incyclefalse
							\aftergroup\CF@chemfig@vi
							\def\CF@next@action{\expandafter\CF@chemfig@v\expandafter{\CF@sub@mol}}%
					\fi
					}%
					{\ifx\CF@remain@molecule\@empty
						\let\CF@next@action\endgroup
					\else% ce qui reste apr\`es le noeud courant n'est pas vide, ne commence pas par "-=~", ni par une parenth\`ese
						\CF@ifx*\CF@toks@a% un cycle ?
						{\ifnum\CF@last@action=\tw@
							\CF@insert@emptygroup\CF@remain@molecule% ins\`ere un groupe vide
						\else
							\ifCF@incycle\let\CF@last@action\thr@@\fi% on \'etait dans un cycle
							\ifnum\CF@last@action=\thr@@\let\CF@lastcycle@num\CF@cycle@num\fi
							\CF@expafterarg@ntimes2\CF@if@firsttokmatch{\expandafter\@gobble\CF@remain@molecule}*% un 2\`e "*" ?
								{\CF@expafterarg@ntimes2{\def\CF@remain@molecule}{\expandafter\@gobble\CF@remain@molecule}% enl\`eve la 1er \'etoile
								\CF@expafterarg@ntimes2\CF@if@firsttokmatch{\expandafter\@gobble\CF@remain@molecule}[% un crochet ensuite ?
									{\expandafter\CF@cycle@parsepreamblewithoptarg\CF@remain@molecule\@nil% \begingroup inclus
									}%
									{\def\CF@cyclearc@startangle{0}\def\CF@cyclearc@endangle{360}%
									\let\CF@cyclearc@directtikz\@empty
									\expandafter\CF@cycle@parsepreamble\CF@remain@molecule\@nil% \begingroup inclus
									}%
								\CF@cyclearctrue
								}%
								{\expandafter\CF@cycle@parsepreamble\CF@remain@molecule\@nil% \begingroup inclus
								\CF@cyclearcfalse
								}%
							\CF@cnt@cycle\z@
							\edef\CF@hook@cycle{\CF@bond@outnode}%
							\let\CF@hook@atomgroup\CF@previous@atomgroup
							\ifx\CF@hook@atomgroup\CF@empty@node
								\let\CF@cycle@joinlast\@ne% joindre le dernier
							\else
								\let\CF@cycle@joinlast\z@
							\fi
							\CF@incycletrue
							\ifnum\CF@last@action=\thr@@
								\pgfmathparse{360/\CF@lastcycle@num-180}% c'est un cycle dans un cycle
							\else
								\pgfmathparse{-180/\CF@cycle@num-90+\CF@cycle@anglecorrection}%
							\fi
							\let\CF@initcycle@angle\pgfmathresult
							\aftergroup\CF@chemfig@vi
							\def\CF@next@action{\expandafter\CF@chemfig@v\expandafter{\CF@sub@mol}}%
						\fi
						}%
						{\errmessage{Package \CF@package@name\space Error: something went wrong here: \detokenize\expandafter{\CF@remain@molecule}^^JIf you think it's a bug, please, send a Minimal Example to the author.}}%
					\fi}%
				}%
		\else
			\CF@expand@second{\CF@expand@second{\CF@expand@second\CF@draw@atomgroup\CF@current@angle}\CF@current@toatom}\CF@current@atomgroup
		\fi
	\fi
	\CF@next@action
}

\CF@def\CF@cycle@parsepreamble*#1#2\@nil{%
	\ifnum#1<\thr@@
		\errmessage{Package \CF@package@name\space Error: A cycle must be at least a triangle.^^JThe number following "*" must be 3 or more}%
	\fi
	\def\CF@remain@molecule{#2}%
	\expandafter\CF@grab@submol\expandafter{\CF@remain@molecule}%
	\begingroup
	\def\CF@cycle@num{#1}%
}

\CF@def\CF@cycle@parsepreamblewithoptarg*[#1]#2#3\@nil{%
	\CF@cycle@parseoptarg#1,\@empty,\@empty,\@empty\@nil
	\CF@cycle@parsepreamble*#2#3\@nil
}

\CF@def\CF@cycle@parseoptarg#1,#2,#3\@nil{%
	\ifx\@empty#1\@empty\def\CF@cyclearc@startangle{0}\else\def\CF@cyclearc@startangle{#1}\fi
	\ifx\@empty#2\@empty\def\CF@cyclearc@endangle{360}\else\def\CF@cyclearc@endangle{#2}\fi
	\expandafter\def\expandafter\CF@cyclearc@directtikz\expandafter{\CF@sanitize@lastitem#3,\@empty\@nil}%
}

\CF@def\CF@grab@submol#1{%
	\begingroup
		\catcode`(\@ne\catcode`)\tw@
		\expandafter\expandafter\expandafter
	\endgroup
	\expandafter\CF@grab@submol@i\scantokens{\relax#1}% le \relax sert \`a meubler pour ne pas que l'argument d\'elimit\'e n'enl\`eve les accolades
}

\CF@def\CF@grab@submol@i#1\@nil{%
	\expandafter\assign@tonil\expandafter\CF@remain@molecule\scantokens\expandafter\expandafter\expandafter{\expandafter\@gobble\@gobble#1}%
	\expandafter\assign@tonil\expandafter\CF@sub@mol\scantokens\expandafter\expandafter\expandafter{\expandafter\@car\@gobble#1\@nil}%
}

\CF@def\assign@tonil#1#2\@nil{\def#1{#2}}

\CF@def\CF@ifcar@isupperletter#1{%
	\ifcat\relax\noexpand#1%
		\let\CF@next\@secondoftwo% faux si c'est une sc
	\else
		\ifnum`#1<`A
			\let\CF@next\@secondoftwo
		\else
			\ifnum`#1>`Z
				\let\CF@next\@secondoftwo
			\else
				\let\CF@next\@firstoftwo
			\fi
		\fi
	\fi
	\CF@next
}

% Cr\'e\'e 4 noeuds au dessus et au dessous des noeuds #1 et #2
% \`a une distance de #3 du noeud #1 et #4 du noeud #2
\CF@def\CF@create@normnodes#1#2#3#4{%
	\ifx\@empty#3\@empty\else
		\node[at=(#1),xshift=#3*\CF@norm@x,yshift=#3*\CF@norm@y](#11){};
		\node[at=(#1),xshift=-#3*\CF@norm@x,yshift=-#3*\CF@norm@y](#12){};
	\fi
	\ifx\@empty#4\@empty\else
		\node[at=(#2),xshift=#4*\CF@norm@x,yshift=#4*\CF@norm@y](#21){};
		\node[at=(#2),xshift=-#4*\CF@norm@x,yshift=-#4*\CF@norm@y](#22){};
	\fi
}

\CF@def\CF@compute@nodevect#1#2{%
	\pgfextractx\CF@dim{\pgfpointanchor{#1}{center}}\edef\CF@dimax{\the\CF@dim}%
	\pgfextracty\CF@dim{\pgfpointanchor{#1}{center}}\edef\CF@dimay{\the\CF@dim}%
	\pgfextractx\CF@dim{\pgfpointanchor{#2}{center}}\edef\CF@dimbx{\the\CF@dim}%
	\pgfextracty\CF@dim{\pgfpointanchor{#2}{center}}\edef\CF@dimby{\the\CF@dim}%
	\pgfmathparse{veclen(\CF@dimbx-\CF@dimax,\CF@dimby-\CF@dimay)}\let\CF@len@vector\pgfmathresult
	\pgfmathparse{(\CF@dimay-\CF@dimby)/\CF@len@vector}\let\CF@norm@x\pgfmathresult
	\pgfmathparse{(\CF@dimbx-\CF@dimax)/\CF@len@vector}\let\CF@norm@y\pgfmathresult
}

\CF@def\CF@set@offset#1#2{%
	\ifx#1\@empty
		\edef#1{\ifx#2\CF@empty@node0pt\else\ifx#2\@empty0pt\else\CF@bond@offset\fi\fi}%
	\fi
}

\CF@def\CF@draw@bond#1#2#3#4#5{% #1=type de liaison #2 et #3:nom de noeuds de d\'ebut et fin #4 et #5: contenu des atomes de d\'ebut et fin
	\CF@set@offset\CF@start@offset#4%
	\CF@set@offset\CF@end@offset#5%
	\let\CF@current@bondstyle\CF@bond@style
	\unless\ifx\CF@current@tikz\@empty\CF@expadd@tocs\CF@current@bondstyle{\expandafter,\CF@current@tikz}\fi
	\path(#2)--(#3)coordinate[pos=0](#2@)coordinate[pos=1](#3@);%
	\CF@compute@nodevect{#2@}{#3@}%
	\pgfmathparse{\CF@start@offset/\CF@len@vector}\let\CF@start@coeff\pgfmathresult
	\pgfmathparse{1-\CF@end@offset/\CF@len@vector}\let\CF@end@coeff\pgfmathresult
	\path(#2@)--(#3@)coordinate[pos=\CF@start@coeff](#2@@)coordinate[pos=\CF@end@coeff](#3@@);%
	\unless\ifx\CF@movebond@name\@empty% on doit poser un noeud sur la liaison
		\path(#2@@)--(#3@@)coordinate[overlay,pos=\CF@movebond@coeff](\CF@movebond@name);
		\let\CF@movebond@name\@empty
	\fi
	\ifcase#1\relax
		\errmessage{Package \CF@package@name\space Error: unknown bond type, this error should not occur^^JIf you think it's a bug, send a Minimal Example to the author}%
	\or% 1 = liaison simple
		\CF@draw@axisbond{#2}{#3}% trace la liaison simple dans l'axe
	\or% 2 = liaison double
		\ifCF@incycle
			\ifnum\CF@doublebond@type=\z@
				\let\CF@doublebond@type\@ne
			\fi
			\ifnum\CF@split@state>\z@
				\let\CF@doublebond@type\tw@
			\fi
			\pgfmathparse{\CF@double@sep*tan(180/\CF@cycle@num)}%
			\let\CF@doublebond@lengthcorrection\pgfmathresult
		\fi
		\ifcase\CF@doublebond@type
			\CF@create@normnodes{#2@@}{#3@@}{\CF@double@sep/2}{\CF@double@sep/2}%
			\CF@draw@bond@i(#2@@1)--(#3@@1);
			\CF@draw@bond@i(#2@@2)--(#3@@2);
			\let\CF@joinbond\z@
		\or
			\CF@create@normnodes{#2@@}{#3@@}\CF@double@sep\CF@double@sep
			\CF@draw@axisbond{#2}{#3}% trace la liaison simple dans l'axe\CF@draw@bond@i(#2@@)--(#3@@);
			\begingroup% ajuste \'eventuellement les longueurs des liaisons doubles
				\ifCF@incycle
					\ifdim\CF@start@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten <=\CF@doublebond@lengthcorrection pt}%
					\fi
					\ifdim\CF@end@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten >=\CF@doublebond@lengthcorrection pt}%
					\fi
				\fi
				\CF@draw@bond@i(#2@@1)--(#3@@1);
			\endgroup
		\or
			\CF@create@normnodes{#2@@}{#3@@}\CF@double@sep\CF@double@sep
			\CF@draw@axisbond{#2}{#3}% trace la liaison simple dans l'axe\CF@draw@bond@i(#2@@)--(#3@@);
			\begingroup% ajuste \'eventuellement les longueurs des liaisons doubles
				\ifCF@incycle
					\ifdim\CF@start@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten \ifnum\CF@split@state=\z@<=-\else>=\fi\CF@doublebond@lengthcorrection pt}%
					\fi
					\ifdim\CF@end@offset=\z@
						\CF@edefadd@tocs\CF@current@bondstyle{,shorten \ifnum\CF@split@state=\z@>=-\else<=\fi\CF@doublebond@lengthcorrection pt}%
					\fi
				\fi
				\CF@draw@bond@i(#2@@2)--(#3@@2);
			\endgroup
		\fi
	\or% 3 = liaison triple
		\CF@create@normnodes{#2@@}{#3@@}\CF@double@sep\CF@double@sep
		\CF@draw@axisbond{#2}{#3}% trace la liaison simple dans l'axe\CF@draw@bond@i(#2@@)--(#3@@);
		\CF@draw@bond@i(#2@@1)--(#3@@1);
		\CF@draw@bond@i(#2@@2)--(#3@@2);
	\or% 4 = liaison Cram pleine de #2 vers #3
		\CF@create@normnodes{#2@@}{#3@@}{\CF@cram@basewidth/2}{}%
		\expandafter\filldraw\expandafter[\CF@current@bondstyle,line join=bevel](#2@@1)--(#2@@2)--(#3@@)--(#2@@1);
		\let\CF@joinbond\z@
	\or% 5 = liaison Cram creuse de #3 vers #2
		\CF@create@normnodes{#3@@}{#2@@}{\CF@cram@basewidth/2}{}%
		\expandafter\filldraw\expandafter[\CF@current@bondstyle,line join=bevel](#3@@1)--(#3@@2)--(#2@@)--(#3@@1);
		\let\CF@joinbond\z@
	\or% 6 = liaison Cram pointill\'ee de #2 vers #3
		\scope
			\CF@create@normnodes{#2@@}{#3@@}{\CF@cram@basewidth/2}{}%
			\clip(#2@@1)--(#2@@2)--(#3@@)--(#2@@1);
			\expandafter\draw\expandafter[\CF@current@bondstyle,dash pattern=on \CF@cram@dashlength off \CF@cram@dashsep,line width=\CF@cram@basewidth](#2@@)--(#3@@);
		\endscope
		\let\CF@joinbond\z@
	\or% 7 = liaison Cram pointill\'ee de #3 vers #2
		\scope
			\CF@create@normnodes{#3@@}{#2@@}{\CF@cram@basewidth/2}{}%
			\clip(#3@@1)--(#3@@2)--(#2@@)--(#3@@1);
			\expandafter\draw\expandafter[\CF@current@bondstyle,dash pattern=on \CF@cram@dashlength off \CF@cram@dashsep,line width=\CF@cram@basewidth](#3@@)--(#2@@);
		\endscope
		\let\CF@joinbond\z@
	\or% 8 = liaison Cram triangle \'evid\'e de #2 vers #3
		\CF@create@normnodes{#2@@}{#3@@}{\CF@cram@basewidth/2}{}%
		\expandafter\draw\expandafter[\CF@current@bondstyle,line join=bevel](#2@@1)--(#2@@2)--(#3@@)--(#2@@1);
		\let\CF@joinbond\z@
	\or% 9 = liaison Cram triangle \'evid\'e de #3 vers #1
		\CF@create@normnodes{#3@@}{#2@@}{\CF@cram@basewidth/2}{}%
		\expandafter\draw\expandafter[\CF@current@bondstyle,line join=bevel](#3@@1)--(#3@@2)--(#2@@)--(#3@@1);
		\let\CF@joinbond\z@
	\else
		\errmessage{Package \CF@package@name\space Error: unknown bond type, this error should not occur^^JIf you think it's a bug, send a Minimal Example to the author}%
	\fi
	\let\CF@start@offset\@empty
	\let\CF@end@offset\@empty
 	\let\CF@previous@tikz\CF@current@tikz
	\let\CF@previous@bondangle\CF@previous@angle
	\def\CF@previous@bond{#1}%
}


\CF@def\CF@draw@axisbond@nojoin#1#2{\CF@draw@bond@i(#1@@)--(#2@@);}

\CF@def\CF@draw@axisbond@join#1#2{% dessine une liaison simple dans l'axe avec raccord rétrograde
	\ifCF@incycle\ifnum\CF@cnt@cycle=\CF@cycle@num\relax\let\CF@next@tikz\CF@cycle@firsttikz\fi\fi
	\ifnum\CF@joinbond=\z@
		\ifCF@incycle
			\ifnum\CF@cnt@cycle=\CF@cycle@num\relax
				\ifnum\CF@cycle@joinlast=\@ne
					\CF@draw@bond@i(#1@@)--(#2@@)--%
						([shift=(\CF@previous@bondangle+2*\CF@cycle@increment@angle:.5\pgflinewidth)]#2@@);
				\else
					\CF@draw@bond@i(#1@@)--(#2@@);
				\fi
			\else
				\CF@draw@bond@i(#1@@)--(#2@@);
			\fi
		\else
			\CF@draw@bond@i(#1@@)--(#2@@);
		\fi
		\let\CF@joinbond\@ne
	\else
		\ifx\CF@previous@tikz\CF@current@tikz
			\let\CF@joinbond\@ne
			\ifx\CF@previous@atomgroup\CF@empty@node
				\ifx\CF@previous@bondangle\empty% si d\'ebut mol\'ecule
					\CF@draw@bond@i(#1@@)--(#2@@);
				\else
					\ifdim\CF@start@offset=\z@
						\ifCF@incycle
							\ifnum\CF@cnt@cycle=\CF@cycle@num\relax
								\ifnum\CF@cycle@joinlast=\@ne
									\ifx\CF@cycle@firsttikz\CF@current@tikz
										\CF@draw@bond@i([shift=(\CF@previous@bondangle:-.5\pgflinewidth)]#1@@)--(#1@@)--(#2@@)--%
										([shift=(\CF@previous@bondangle+2*\CF@cycle@increment@angle:.5\pgflinewidth)]#2@@);
									\else
										\CF@draw@bond@i([shift=(\CF@previous@bondangle:-.5\pgflinewidth)]#1@@)--(#1@@)--(#2@@);
									\fi
								\else
									\CF@draw@bond@i([shift=(\CF@previous@bondangle:-.5\pgflinewidth)]#1@@)--(#1@@)--(#2@@);
								\fi
							\else
								\CF@draw@bond@i([shift=(\CF@previous@bondangle:-.5\pgflinewidth)]#1@@)--(#1@@)--(#2@@);
							\fi
						\else
							\CF@draw@bond@i([shift=(\CF@previous@bondangle:-.5\pgflinewidth)]#1@@)--(#1@@)--(#2@@);
						\fi
					\else
						\CF@draw@bond@i(#1@@)--(#2@@);
					\fi
				\fi
			\else
				\CF@draw@bond@i(#1@@)--(#2@@);
			\fi
		\else
			\ifCF@incycle
				\ifnum\CF@cnt@cycle=\CF@cycle@num\relax
					\ifnum\CF@cycle@joinlast=\@ne
						\ifx\CF@next@tikz\CF@current@tikz
							\CF@draw@bond@i(#1@@)--(#2@@)--%
								([shift=(\CF@previous@bondangle+2*\CF@cycle@increment@angle:.5\pgflinewidth)]#2@@);
						\else
							\CF@draw@bond@i(#1@@)--(#2@@);
						\fi
					\else
						\CF@draw@bond@i(#1@@)--(#2@@);
					\fi
				\else
					\CF@draw@bond@i(#1@@)--(#2@@);
				\fi
			\else
				\CF@draw@bond@i(#1@@)--(#2@@);
			\fi
		\fi
 	\fi
 	\ifdim\CF@end@offset=\z@\else\let\CF@joinbond\z@\fi
}

\CF@def\enablebondjoin {\global\let\CF@draw@axisbond\CF@draw@axisbond@join}
\CF@def\disablebondjoin{\global\let\CF@draw@axisbond\CF@draw@axisbond@nojoin}
\disablebondjoin% par d\'efaut, d\'esactiver la jointure entre liaisons

\CF@def\CF@draw@bond@i{\expandafter\draw\expandafter[\CF@current@bondstyle]}

\CF@def\CF@hook@drawall{% dessine tous les crochets contenus dans la sc \CF@hook@draw
	\unless\ifx\CF@hook@drawlist\@empty
		\expandafter\CF@hook@drawfirst\CF@hook@drawlist\@nil% trace un lien de crochet \`a crochet
		\expandafter\CF@hook@drawall
	\fi
}

\CF@def\CF@hook@drawfirst[#1,#2,#3]#4#5#6#7#8\@nil{%
	\def\CF@hook@drawlist{#8}%
	\begingroup
		\let\CF@joinbond\z@
		\def\CF@current@tikz{#3}%
		\def\CF@hook@startcontent{#6}\def\CF@hook@endcontent{#7}%
		\CF@if@integer{#2}%
			{\CF@draw@bond{#2}{#4}{#5}\CF@hook@startcontent\CF@hook@endcontent}%
			{\CF@bond@findcode{#2}\CF@bond@currentnum
			\CF@draw@bond\CF@bond@currentnum{#4}{#5}\CF@hook@startcontent\CF@hook@endcontent
			}%
	\endgroup
}

\CF@def\CF@extract@atom#1-#2\@nil{#2}% transforme le bound@outnode en n° de l'atome

\CF@def\setnodestyle{\def\CF@node@style}
\setnodestyle{}

\CF@def\setbondstyle{\def\CF@bond@style}
\setbondstyle{}

\expandafter\CF@def\expandafter\CF@gobble@movearg\string @#1#2\@nil#3{%
	\expandafter\def\csname atom@\number\CF@cnt@atomnumber\endcsname{#2}%
	\CF@if@instr{#1},%
		{\CF@analyse@movearg#1\@nil#3\let\CF@movebond@coeff\@empty}%
		{\def#3{#1}}%
	\ifx\@empty#2\@empty\let\CF@node@strut\@empty\fi
}%

\CF@def\hflipnext{\let\CF@split@state\@ne}

\CF@def\vflipnext{\let\CF@split@state\tw@}
\let\CF@split@state\z@

\CF@def\CF@draw@atomgroup#1#2#3{% #1=angle d'arriv\'ee de la liaison #2=numero atome sur lequel arrive la liaison #3=groupe d'atomes
	\expandafter\let\expandafter\CF@bond@outcontent% assigne le contenu de l'atome d'o\`u part la liaison
		\csname
			\ifdefined\CF@bond@outnode
				atom@\expandafter\CF@extract@atom\CF@bond@outnode\@nil
			\else
				@empty%
			\fi
		\endcsname
	\global\advance\CF@cnt@groupnumber\@ne
	\let\CF@current@atom\@empty
	\global\let\CF@hook@drawlist\@empty
	\CF@cnt@atomingroup\z@
	\CF@if@firsttokmatch{#3}?{\CF@draw@atomgroup@i{{}#3}}{\CF@draw@atomgroup@i{#3}}%
	\def\CF@current@atomgroup{#3}%
	\CF@remove@movearg\CF@current@atomgroup% enl\`eve les "@{<nom>}"
	\CF@if@instr{#3}?%
		{\CF@remove@hook\CF@current@atomgroup
		\ifcat\relax\detokenize\expandafter{\romannumeral-`\.\expandafter\noexpand\CF@current@atomgroup}\relax
			\let\CF@current@atomgroup\CF@empty@node
		\fi
		}%
		\relax
	\ifx\@empty#2\@empty
	\else
		\ifnum#2<\@ne
			\immediate\write\CF@unused{Package \CF@package@name\space Warning: no atom found at position #2, pershaps you mispelled the optional argument of the bond.}%
		\else
			\ifnum#2>\CF@cnt@atomingroup
				\errmessage{Package \CF@package@name\space Error: no atom found at position #2, pershaps you mispelled the optional argument of the bond.}%
			\fi
		\fi
	\fi
	\edef\CF@hook@atomnumber{%
		\ifx\@empty#2\@empty
			\ifdim#1pt>90pt
				\ifdim#1pt<270pt \number\CF@cnt@atomingroup\else1\fi
			\else1%
			\fi
		\else#2%
		\fi}%
	\CF@cnt@atomnumber\CF@hook@atomnumber
	\ifx\CF@current@atomgroup\CF@empty@node
		\let\CF@node@strut\@empty
	\else
		\ifx\@empty\CF@bond@outcontentsaved
			\def\CF@node@strut{\vphantom\CF@bond@outcontent}%
		\else
			\def\CF@node@strut{\vphantom\CF@bond@outcontentsaved}%
		\fi
	\fi
	\edef\CF@opt@string{anchor=\ifnum\CF@last@action=\z@ base\else\ifCF@incycle center\else\ifCF@macrofixedbondlength 180+#1\else center\fi\fi\fi,at=(CF@node),\CF@node@style}% premier atome de la mol\'ecule affich\'e
	\loop
		\unless\ifnum\CF@cnt@atomnumber>\CF@cnt@atomingroup
		\expandafter\expandafter\expandafter\futurelet\expandafter\expandafter\expandafter\CF@toks@a\expandafter\expandafter\expandafter
			\CF@gobble@tonil\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil
		\expandafter\ifx\string @\CF@toks@a% l'atome courant commence par un "@"
			\expandafter\expandafter\expandafter\CF@gobble@movearg\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil\CF@moveatom@name
			\expandafter\node\expandafter[\CF@opt@string,overlay](\CF@moveatom@name){\phantom{\CF@node@content}};%
			\let\CF@moveatom@name\@empty
		\fi
		\expandafter\node\expandafter[\CF@opt@string](n\number\CF@cnt@groupnumber-\number\CF@cnt@atomnumber){\CF@node@content};%
		\let\CF@node@strut\@empty
		\advance\CF@cnt@atomnumber\@ne
		\edef\CF@opt@string{anchor=base \ifnum\CF@split@state=\@ne east\else west\fi,at=(n\number\CF@cnt@groupnumber-\number\numexpr\CF@cnt@atomnumber-1.base \ifnum\CF@split@state=\@ne west\else east\fi),\CF@node@style}%
	\repeat
	\CF@cnt@atomnumber\CF@hook@atomnumber
	\ifnum\CF@last@action=\tw@% s'il faut tracer une liaison
		\gdef\CF@cycle@anglecorrection{0}% alors c'est qu'un cycle ne peut pas commencer la mol\'ecule : annulation de la correction d'angle
		\CF@draw@bond\CF@bond@type{\CF@bond@outnode}{n\number\CF@cnt@groupnumber-\number\CF@cnt@atomnumber}\CF@previous@atomgroup\CF@current@atomgroup
	\fi
	\let\CF@last@action\@ne% met la derni\`ere action \`a 1 : affichage d'un noeud
	\loop
		\ifnum\CF@cnt@atomnumber>\@ne
		\advance\CF@cnt@atomnumber\m@ne
		\edef\CF@opt@string{anchor=base \ifnum\CF@split@state=\@ne west\else east\fi,at=(n\number\CF@cnt@groupnumber-\number\numexpr\CF@cnt@atomnumber+1.base \ifnum\CF@split@state=\@ne east\else west\fi),\CF@node@style}%
		\expandafter\expandafter\expandafter\futurelet\expandafter\expandafter\expandafter\CF@toks@a\expandafter\expandafter\expandafter
			\CF@gobble@tonil\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil
		\expandafter\ifx\string @\CF@toks@a% l'atome courant commence par un "@"
			\expandafter\expandafter\expandafter\CF@gobble@movearg\csname atom@\number\CF@cnt@atomnumber\endcsname\@nil\CF@moveatom@name
			\expandafter\node\expandafter[\CF@opt@string,overlay](\CF@moveatom@name){\phantom{\CF@node@content}};%
			\let\CF@moveatom@name\@empty
		\fi
		\expandafter\node\expandafter[\CF@opt@string](n\number\CF@cnt@groupnumber-\number\CF@cnt@atomnumber){\CF@node@content};%
	\repeat
	\CF@hook@drawall
	\edef\CF@last@groupnumber{\number\CF@cnt@groupnumber}%
	\let\CF@previous@atomgroup\CF@current@atomgroup
}

\expandafter\CF@def\expandafter\CF@keep@movearg\string @#1#2\@nil{\expandafter\def\expandafter\CF@current@atom\expandafter{\string @{#1}}}

\CF@def\CF@draw@atomgroup@i#1{% transforme #1 en un groupe d'atomes
	\ifx\@empty#1\@empty
		\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
	\else
		\advance\CF@cnt@atomingroup\@ne
		\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
		\expandafter\CF@ifx\string @\CF@toks@a
			{\CF@keep@movearg#1\@nil
			\CF@swap@fi
			\CF@remove@movearg@i#1\@nil\CF@after@movearg
			\expandafter\CF@draw@atomgroup@ii\expandafter{\CF@after@movearg}%
			}%
			{\CF@swap@fi
			\let\CF@current@atom\@empty
			\CF@draw@atomgroup@ii{#1}%
			}%
	\fi
}

\CF@def\CF@draw@atomgroup@ii#1{%
	\ifx\@empty#1\@empty
		\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
	\else
	\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
	\CF@ifx\bgroup\CF@toks@a
		{\CF@expadd@tocs\CF@current@atom{\expandafter{\@car#1\@nil}}%
		\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
		}%
		{\CF@ifx\@sptoken\CF@toks@a
			{\CF@add@tocs\CF@current@atom{ }%
			\expandafter\CF@draw@atomgroup@iii\expandafter{\CF@after@space#1\@nil}%
			}%
			{\CF@expadd@tocs\CF@current@atom{\@car#1\@nil}%
			\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
			}%
		}%
	\fi
}

% enl\`eve tous les "@{nom}" de la sc #1
\CF@def\CF@remove@movearg#1{%
	\CF@expand@afterfirst{\expandafter\CF@if@instr\expandafter{#1}}{\string @}%
		{\expandafter\CF@remove@movearg@i#1\@nil#1%
		\CF@remove@movearg#1}%
		\relax
}

% enl\`eve le premier "@{<nom>}" de l'argument et l'assigne \`a #2
\CF@def\CF@remove@movearg@i#1\@nil#2{%
	\expandafter\def\expandafter\CF@remove@movearg@ii\expandafter##\expandafter1\string @{%
		\expandafter\def\expandafter#2\expandafter{\@gobble##1}% mange le \relax
		\CF@remove@movearg@iii\relax
	}%
	\def\CF@remove@movearg@iii##1\@nil{\CF@expadd@tocs#2{\@gobbletwo##1}}% mange le \relax et le <nom>
	\CF@remove@movearg@ii\relax#1\@nil
}

\CF@def\CF@draw@atomgroup@iii#1{% transforme #1 en un groupe d'atomes
	\ifx\@empty#1\@empty%
		\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
		\let\CF@current@atom\@empty
	\else
		\futurelet\CF@toks@a\CF@gobble@tonil#1\@nil
		\expandafter\CF@ifx\string @\CF@toks@a
			{\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
			\let\CF@current@atom\@empty
			\CF@swap@fi\CF@draw@atomgroup@i{#1}%
			}%
			{\CF@ifx|\CF@toks@a
				{\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
				\let\CF@current@atom\@empty
				\CF@swap@fi\expandafter\CF@draw@atomgroup@i\expandafter{\@gobble#1}%
				}%
				{\CF@ifx\@sptoken\CF@toks@a
					{\CF@add@tocs\CF@current@atom{ }%
					\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\CF@after@space#1\@nil}%
					 }%
					{\CF@ifx\bgroup\CF@toks@a
						{\CF@expadd@tocs\CF@current@atom{\expandafter{\@car#1\@nil}}%
						\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
						}%
						{\expandafter\CF@ifcar@isupperletter\expandafter{\@car#1\@nil}%
							{\expandafter\let\csname atom@\number\CF@cnt@atomingroup\endcsname\CF@current@atom
							\let\CF@current@atom\@empty
							\CF@swap@fi\CF@draw@atomgroup@i{#1}%
							}%
							{\CF@ifx?\CF@toks@a
								{\expandafter\CF@if@firsttokmatch\expandafter{\@gobble#1}[% un crochet apr\`es le "?"
									{\expandafter\CF@grab@optarg\@gobble#1\@nil\CF@after@hook}%
									{\expandafter\CF@grab@optarg\expandafter[\expandafter]\@gobble#1\@nil\CF@after@hook}%
									\CF@expand@second{\CF@expand@second\CF@if@instr\CF@hook@list}{\expandafter(\CF@hook@currentname)}% crochet d\'ej\`a d\'efini ?
									{\expandafter\CF@hook@parselist\expandafter{\CF@hook@currentname}% va chercher les caract\'eristiques du crochet sauvegard\'e
									\CF@edefadd@tocs\CF@hook@drawlist{%
										[\CF@hook@currentname,\CF@hook@currentlink,\CF@hook@currenttikz]{\CF@hook@savedcoord}{n\number\CF@cnt@groupnumber-\number\CF@cnt@atomingroup}}%
									\CF@expadd@tocs\CF@hook@drawlist{\expandafter{\CF@hook@savedcontent}}%
									\CF@expadd@tocs\CF@hook@drawlist{\expandafter{\CF@current@atom}}% ajoute les 4 arguments \`a la liste des crochets \`a tracer
									\global\let\CF@hook@drawlist\CF@hook@drawlist
									}%
									{\CF@edefadd@tocs\CF@hook@list{(\CF@hook@currentname)|n\number\CF@cnt@groupnumber-\number\CF@cnt@atomingroup|}%
									\CF@expadd@tocs\CF@hook@list{\CF@current@atom|}%
									\global\let\CF@hook@list\CF@hook@list
									}%
								\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\CF@after@hook}%
								}%
								{\CF@expadd@tocs\CF@current@atom{\@car#1\@nil}%
								\CF@swap@fi\expandafter\CF@draw@atomgroup@iii\expandafter{\@gobble#1}%
								}%
							}%
						}%
					}%
				}%
			}%
	\fi
}

\CF@def\CF@kook@defaultname{a}
\CF@def\CF@hook@defaultlink{-}
\CF@def\CF@hook@defaulttikz{}

\CF@def\CF@hook@parseoptarg#1,#2,#3\@nil{%
	\CF@testempty@andassign\CF@hook@currentname{#1}\CF@kook@defaultname
	\CF@testempty@andassign\CF@hook@currentlink{#2}\CF@hook@defaultlink
	\CF@testempty@andassign\CF@hook@currenttikz{#3}\CF@hook@defaulttikz
}

\CF@def\CF@grab@optarg[#1]#2\@nil#3{%
	\CF@hook@parseoptarg#1,,\@nil
	\def#3{#2}%
}

\CF@def\CF@hook@parselist#1{% #1 est le nom du noeud \`a retrouver
	\def\CF@hook@parselist@i##1(#1)|##2|##3|##4\@nil{\def\CF@hook@savedcoord{##2}\def\CF@hook@savedcontent{##3}}%
	\expandafter\CF@hook@parselist@i\CF@hook@list\@nil
}

\CF@def\CF@remove@hook#1{%
	\expandafter\CF@if@instr\expandafter{#1}?%
		{\expandafter\CF@remove@hook@i\expandafter\relax#1\@nil#1%
		\CF@remove@hook#1%
		}
		\relax
}

\CF@def\CF@remove@hook@i#1?#2\@nil#3{%
	\CF@if@firsttokmatch{#2}[%
		{\CF@remove@hook@ii#1?#2\@nil#3}
		{\expandafter\def\expandafter#3\expandafter{\@gobble#1#2}}%
}

\CF@def\CF@remove@hook@ii#1?[#2]#3\@nil#4{\expandafter\def\expandafter#4\expandafter{\@gobble#1#3}}

\CF@def\setlewis{\@testopt\CF@setlewis{0.3ex}}

\CF@def\CF@setlewis[#1]#2#3#4{%
	\def\CF@lewis@widthdouble{#1}%
	\ifx\@empty#2\@empty\def\CF@lewis@offset{0.4ex}\else\def\CF@lewis@offset{#2}\fi
	\ifx\@empty#3\@empty\def\CF@lewis@length{1.5ex}\else\def\CF@lewis@length{#3}\fi
	\ifx\@empty#4\@empty\def\CF@lewis@style{}\else\def\CF@lewis@style{#4}\fi
}
\setlewis{}{}{}

\CF@def\setlewisdist#1{%
	\def\CF@lewis@dist{#1}\ifx\@empty\CF@lewis@dist\def\CF@lewis@dist{0.2em}\fi
}
\setlewisdist{0.3em}

\CF@def\Lewis{\@testopt{\CF@lewis@i{}}{1}}

\CF@def\lewis{\@testopt{\CF@lewis@i{,overlay}}{1}}

\CF@def\CF@lewis@i#1[#2]{%
	\def\CF@lewis@diagcoeff{#2}%
	\ifx\@empty\CF@lewis@diagcoeff\def\CF@lewis@diagcoeff{1}\fi
	\CF@lewis@ii{#1}%
}

\CF@def\CF@lewis@ii#1#2{\CF@lewis@iii#2\@nil{#1}}

\CF@def\CF@lewis@iii#1,#2\@nil#3{%
	\setbox\CF@lewis@box\hbox{\printatom{#2}}% mettre en dehors de tikzpicture (si \printatom ne passe pas en mode math)
	\tikzpicture[every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline]%
		\@makeother;\@makeother:%
		\node(CF@lewis@anchor){};
		\def\CF@lewis@remainpos{#1}%
		\let\CF@lewis@previouspos\@empty
		\loop
			\unless\ifx\CF@lewis@remainpos\@empty
				\edef\CF@lewis@currentpos{\expandafter\@car\CF@lewis@remainpos\@nil}%
				\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
				\pgfmathparse{\wd\CF@lewis@box/2+\ifcase\CF@lewis@currentpos\space1\or1\or0\or-1\or-1\or-1\or0\or1\fi*(\wd\CF@lewis@box/2)}%
				\let\CF@lewis@x\pgfmathresult
				\pgfmathparse{\ht\CF@lewis@box/2+\ifcase\CF@lewis@currentpos\space0\or1\or1\or1\or0\or-1\or-1\or-1\fi*(\ht\CF@lewis@box/2\ifnum\CF@lewis@currentpos>4 +\dp\CF@lewis@box\fi)}%
				\let\CF@lewis@y\pgfmathresult
				\edef\CF@lewis@xoffset{\ifcase\CF@lewis@currentpos\space1\or0.70711\or0\or-0.70711\or-1\or-0.70711\or0\or0.70711\fi}%
				\edef\CF@lewis@yoffset{\ifcase\CF@lewis@currentpos\space0\or0.70711\or1\or0.70711\or0\or-0.70711\or-1\or-0.70711\fi}%
				\ifodd\CF@lewis@currentpos\relax
					\pgfmathparse{\CF@lewis@offset*\CF@lewis@diagcoeff}\let\CF@lewis@current@offset\pgfmathresult
				\else
					\let\CF@lewis@current@offset\CF@lewis@offset
				\fi
				\if.\expandafter\@car\CF@lewis@remainpos\relax\@nil
					\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
					\CF@expand@afterfirst{\draw[fill,black,}{\CF@lewis@style#3]}%
						(\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset,\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset)circle(0.15ex);%
				\else
					\if|\expandafter\@car\CF@lewis@remainpos\relax\@nil
						\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
						\pgfmathparse{\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset}\let\CF@lewis@x\pgfmathresult
						\pgfmathparse{\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset}\let\CF@lewis@y\pgfmathresult
						\expandafter\draw\expandafter[\CF@lewis@style#3]%
							(\CF@lewis@x pt+\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y-\CF@lewis@length*\CF@lewis@xoffset/2 pt)--
							(\CF@lewis@x pt+\CF@lewis@length*\CF@lewis@yoffset/2 pt+\CF@lewis@xoffset*\CF@lewis@widthdouble,\CF@lewis@y-\CF@lewis@length*\CF@lewis@xoffset/2 pt+\CF@lewis@yoffset*\CF@lewis@widthdouble)--
							(\CF@lewis@x pt-\CF@lewis@length*\CF@lewis@yoffset/2 pt+\CF@lewis@xoffset*\CF@lewis@widthdouble,\CF@lewis@y+\CF@lewis@length*\CF@lewis@xoffset/2 pt+\CF@lewis@yoffset*\CF@lewis@widthdouble)--
							(\CF@lewis@x pt-\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y+\CF@lewis@length*\CF@lewis@xoffset/2 pt)--cycle;%
					\else
						\if:\expandafter\@car\CF@lewis@remainpos\relax\@nil
							\edef\CF@lewis@remainpos{\expandafter\@gobble\CF@lewis@remainpos}%
							\pgfmathparse{\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset}\let\CF@lewis@x\pgfmathresult
							\pgfmathparse{\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset}\let\CF@lewis@y\pgfmathresult
							\CF@expand@afterfirst{\draw[fill,black,}{\CF@lewis@style#3]}%
								(\CF@lewis@x pt+\CF@lewis@dist*\CF@lewis@yoffset/2 pt,\CF@lewis@y-\CF@lewis@dist*\CF@lewis@xoffset/2 pt)circle(0.15ex)%
								(\CF@lewis@x pt-\CF@lewis@dist*\CF@lewis@yoffset/2 pt,\CF@lewis@y+\CF@lewis@dist*\CF@lewis@xoffset/2 pt)circle(0.15ex);%
						\else
							\pgfmathparse{\CF@lewis@x pt+\CF@lewis@xoffset*\CF@lewis@current@offset}\let\CF@lewis@x\pgfmathresult
							\pgfmathparse{\CF@lewis@y pt+\CF@lewis@yoffset*\CF@lewis@current@offset}\let\CF@lewis@y\pgfmathresult
							\expandafter\draw\expandafter[\CF@lewis@style#3]%
								(\CF@lewis@x pt+\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y-\CF@lewis@length*\CF@lewis@xoffset/2 pt)--%
								(\CF@lewis@x pt-\CF@lewis@length*\CF@lewis@yoffset/2 pt,\CF@lewis@y+\CF@lewis@length*\CF@lewis@xoffset/2 pt);%
						\fi
					\fi
			\fi
		\repeat
		\node[anchor=base west]at(CF@lewis@anchor){\box\CF@lewis@box};%
	\endtikzpicture
}

\CF@def\setstacksep#1{\edef\CF@stacksep{\ifx\@empty#1\@empty1.5pt\else\the\dimexpr#1\relax\fi}}
\setstacksep{1.5pt}

\CF@def\Chembelow{\begingroup\let\CF@tmp@str\@gobble\CF@chembelow@i}

\CF@def\chembelow{\begingroup\let\CF@tmp@str\@firstofone\CF@chembelow@i}

\CF@def\CF@chembelow@i{\@testopt\CF@chembelow@ii\CF@stacksep}

\CF@def\CF@chembelow@ii[#1]#2#3{%
	\setbox\CF@box@boxa\hbox{\printatom{#2}}%
	\expandafter\vtop\CF@tmp@str{to\ht\CF@box@boxa}{%
		\offinterlineskip
		\hbox{\printatom{#2}}%
		\kern#1\relax
		\hbox to\wd\CF@box@boxa{\hss\printatom{#3}\hss}%
		\CF@tmp@str\vss
		}%
	\endgroup
}

\CF@def\Chemabove{\begingroup\let\CF@tmp@str\@gobble\CF@chemabove@i}

\CF@def\chemabove{\begingroup\let\CF@tmp@str\@firstofone\CF@chemabove@i}

\CF@def\CF@chemabove@i{\@testopt\CF@chemabove@ii\CF@stacksep}

\CF@def\CF@chemabove@ii[#1]#2#3{%
	\setbox\CF@box@boxa\hbox{\printatom{#2}}%
	\expandafter\vbox\CF@tmp@str{to\ht\CF@box@boxa}{%
		\offinterlineskip
		\CF@tmp@str\vss
		\hbox to\wd\CF@box@boxa{\hss\printatom{#3}\hss}%
		\kern#1\relax
		\hbox{\printatom{#2}}%
	}%
	\endgroup
}

%%%%%% les signes et les fl\`eches
\CF@def\chemsign{\@testopt\CF@chemsign{0.5em}}

\CF@def\CF@chemsign[#1]#2{\hbox{\kern#1\relax#2\kern#1}}

\CF@def\setchemrel#1#2#3{%
	\ifx\@empty#1\@empty\def\CF@chemrel@vsep{2pt}\else\def\CF@chemrel@vsep{#1}\fi
	\ifx\@empty#2\@empty\def\CF@chemrel@hsep{0.7em}\else\def\CF@chemrel@hsep{#2}\fi
	\ifx\@empty#3\@empty\def\CF@chemrel@length{4em}\else\def\CF@chemrel@length{#3}\fi
}

\setchemrel{}{}{}

\CF@def\chemrel{%
	\immediate\write\CF@unused{Package \CF@package@name\space Warning: the macro \string\chemrel\space is deprecated. Please, build schemes with \string\schemestart\space and inside, use \string\arrow.}%
	\@testopt\CF@chemchemrel@i{}%
}

\CF@def\CF@chemchemrel@i[#1]{\@testopt{\CF@chemchemrel@ii[#1]}{}}

\CF@def\CF@chemchemrel@ii[#1][#2]#3{%
	\def\CF@chemrel@stuff
		{\leavevmode\kern\CF@chemrel@hsep
		\tikzpicture[every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline]%
			\CF@if@instr{#3}{<>}%
				{\node[yshift=-1pt] at(0,0)(chemrel@start){\vphantom I};\node[yshift=-1pt] at(\CF@chemrel@length,0)(chemrel@end){\vphantom I};%
				\expandafter\draw\expandafter[\CF@remove@equichars#3,\@nil-](chemrel@end)--(chemrel@start);\fill (chemrel@start)--++(4pt,-1.75pt)--+(-1.5pt,1.75pt)--cycle;%
				\node[yshift=1pt] at(0,0)(chemrel@start){\vphantom I};\node[yshift=1pt] at(\CF@chemrel@length,0)(chemrel@end){\vphantom I};%
				\expandafter\draw\expandafter[\CF@remove@equichars#3,\@nil-](chemrel@start)--(chemrel@end);\fill(chemrel@end)--++(-4pt,1.75pt)--+(1.5pt,-1.75pt)--cycle;
				}%
				{\node at(0,0)(chemrel@start){\vphantom I};\node at(\CF@chemrel@length,0)(chemrel@end){\vphantom I};%
				\draw[#3](chemrel@start)--(chemrel@end);%
				}%
		\endtikzpicture
		\kern\CF@chemrel@hsep
		}%
	\ifx\@empty#1\@empty
		\ifx\@empty#2\@empty\CF@chemrel@stuff
		\else\chembelow[\CF@chemrel@vsep]\CF@chemrel@stuff{\hbox{#2}}%
		\fi
	\else
		\ifx\@empty#2\@empty\chemabove[\CF@chemrel@vsep]\CF@chemrel@stuff{\hbox{#1}}%
		\else\chemabove[\CF@chemrel@vsep]{\chembelow[\CF@chemrel@vsep]\CF@chemrel@stuff{\hbox{#2}}}{\hbox{#1}}%
		\fi
	\fi
}

\CF@def\CF@remove@equichars#1<>#2\@nil{#1#2}

\CF@def\chemmove{\@testopt\CF@chemmove{}}

\CF@def\CF@chemmove[#1]#2{%
	\ifx\@empty#2\@empty
		\expandafter\@gobble
	\else
		\expandafter\@firstofone
	\fi
	{\expandafter\tikzpicture\romannumeral\CF@ifx{\@empty#1}\@empty
		{\z@[remember picture,overlay]}{\z@[remember picture,overlay,#1]}#2
		\endtikzpicture
	}%
}

\CF@def\chemnameinit#1{%
	\setbox\CF@stuff@box\hbox{#1}%
	\xdef\CF@dp@max{\the\dp\CF@stuff@box}%
}
\let\CF@dp@max\z@

\CF@def\CF@parse@molname#1\\#2\@nil{%
	\hbox to\CF@wd@stuffbox{\hss#1\hss}%
	\ifx\@empty#2\@empty
	\else
		\CF@swap@fi
		\CF@parse@molname#2\@nil
	\fi
}

\CF@def\chemname{%
	\@ifstar
		{\CF@name@dp@adjustfalse\CF@chemnam@i}
		{\CF@name@dp@adjusttrue\CF@chemnam@i}%
}

\CF@def\CF@chemnam@i{\@testopt\CF@chemname@ii{1.5ex}}

\CF@def\CF@chemname@ii[#1]#2#3{%
	\setbox\CF@stuff@box\hbox{#2}%
	\edef\CF@wd@stuffbox{\the\wd\CF@stuff@box}\edef\CF@dp@stuffbox{\the\dp\CF@stuff@box}%
	\leavevmode
	\ifdim\CF@dp@max<\CF@dp@stuffbox\global\let\CF@dp@max\CF@dp@stuffbox\fi
	\vtop{%
		\box\CF@stuff@box
		\nointerlineskip
		\kern\dimexpr#1\ifCF@name@dp@adjust+\CF@dp@max-\CF@dp@stuffbox\fi\relax
		\CF@parse@molname#3\\\@nil
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    S C H E M A S      R E A C T I O N N E L S    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcount\CF@compound@cnt

\newdimen\CF@arrow@size

\newif\ifCF@name@start
\newif\ifCF@name@end
\newif\ifCF@reac@debug

\let\CF@scheme@nest\z@% ne PAS modifier cette ligne !

\CF@def\CF@subscheme{\@testopt\CF@subscheme@i{}}
\CF@def\CF@subscheme@i[#1]{\@testopt{\CF@subscheme@ii[#1]}{text}}
\CF@def\CF@subscheme@ii[#1][#2]#3{\schemestart[#1][#2]#3\schemestop}

\CF@def\schemedebug#1{\ifcsname CF@reac@debug#1\endcsname\csname CF@reac@debug#1\endcsname\else\CF@reac@debugfalse\fi}
\schemedebug{false}

\CF@def\setcompoundstyle{\def\CF@default@compound@style}
\setcompoundstyle{}

\CF@def\CF@set@arrow@style#1,#2,#3\@nil#4#5#6{%
	\def#4{#1}%
	\expandafter\def\expandafter#5\expandafter{#2}%
	\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#6\expandafter\expandafter\expandafter{\expandafter\CF@sanitize@lastitem#3,\@empty\@nil}%
}

\CF@def\setarrowdefault#1{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@default@arrow@angle\CF@default@arrow@length\CF@default@arrow@style
	\ifx\@empty\CF@default@arrow@angle\def\CF@default@arrow@angle{0}\fi
	\ifx\@empty\CF@default@arrow@length\def\CF@default@arrow@length{1}\fi
}
\setarrowdefault{}

\CF@def\setarrowoffset#1{\def\CF@arrow@offset{#1}\ifx\CF@arrow@offset\@empty\def\CF@arrow@offset{1em}\fi}
\setarrowoffset{}

\CF@def\setcompoundsep#1{\def\CF@compound@sep{#1}\ifx\CF@compound@sep\@empty\def\CF@compound@sep{5em}\fi}
\setcompoundsep{}

\CF@def\setarrowlabelsep#1{\def\CF@arrow@labelsep{#1}\ifx\CF@arrow@labelsep\@empty\def\CF@arrow@labelsep{3pt}\fi}
\setarrowlabelsep{}

\CF@def\chemleft#1#2\chemright#3{%
	\leavevmode
	\begingroup
		\setbox\z@\hbox{$\vcenter{\hbox{}}$}\edef\CF@delim@math@ht{\the\ht\z@}%
		\setbox\z@\hbox{#2}\edef\CF@delim@dim{\the\dimexpr(\ht\z@+\dp\z@)/\tw@}%
		\edef\CF@delim@shift{\the\dimexpr(\ht\z@-\dp\z@)/\tw@-\CF@delim@math@ht}%
		\raise\CF@delim@shift\hbox{$\left#1\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right.$}\box\z@
		\raise\CF@delim@shift\hbox{$\left.\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right#3$}%
	\endgroup
}

\CF@def\chemright#1{%
	\immediate\write\CF@unused{Package \CF@package@name\space Warning: "\string\chemright\string#1"ignored! No \string\chemleft\space previously found.^^J}%
}

\CF@def\chemup#1#2\chemdown#3{%
	\begingroup
		\setbox\z@\hbox{\printatom{#2}}\edef\CF@delim@dim{\the\dimexpr\wd\z@/\tw@}%
		\tikzpicture[every node/.style={inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline]%
			\node[anchor=base west](chem@stuff){\box\z@};%
			\node[at=(chem@stuff.north),anchor=east,rotate=-90]{$\left#1\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right.$};%
			\node[at=(chem@stuff.south),anchor=west,rotate=-90]{$\left.\vrule height\CF@delim@dim depth\CF@delim@dim width\z@\right#3$};%
		\endtikzpicture
	\endgroup
}

\CF@def\chemdown#1{%
	\immediate\write\CF@unused{Package \CF@package@name\space Warning: "\string\chemdown\string#1" ignored! No \string\chemup\space previously found.^^J}%
}

\CF@def\CF@and{\futurelet\CF@toks@a\CF@and@i}

\CF@def\CF@and@i{%
	\ifx\CF@toks@a\bgroup
		\expandafter\CF@and@ii
	\else
		\expandafter\CF@and@ii\expandafter{\expandafter}%
	\fi
}

\CF@def\CF@and@ii#1{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@signspace@ante\CF@signspace@post\CF@sign@vshift
	\ifx\@empty\CF@signspace@ante\let\CF@signspace@ante\CF@signspace@ante@default\fi
	\ifx\@empty\CF@signspace@post\let\CF@signspace@post\CF@signspace@post@default\fi
	\ifx\@empty\CF@sign@vshift\let\CF@sign@vshift\CF@sign@vshift@default\fi
	\raise\CF@sign@vshift\hbox{\kern\CF@signspace@ante$+$\kern\CF@signspace@post}%
}

\CF@def\setandsign#1{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@signspace@ante@default\CF@signspace@post@default\CF@sign@vshift@default
	\ifx\@empty\CF@signspace@ante@default\def\CF@signspace@ante@default{.5em}\fi
	\ifx\@empty\CF@signspace@post@default\def\CF@signspace@post@default{.5em}\fi
	\ifx\@empty\CF@sign@vshift@default\let\CF@sign@vshift@default\z@\fi
}
\setandsign{}

\CF@def\schemestart{%
	\xdef\CF@scheme@nest{\number\numexpr\CF@scheme@nest+\@ne}%
	\@testopt\CF@schemestart@i{}%
}

\CF@def\CF@schemestart@i[#1]{%
	\CF@set@arrow@style#1,\@empty,\@empty\@nil\CF@arrow@angle\CF@arrow@length\CF@arrow@style
	\ifx\@empty\CF@arrow@angle\let\CF@arrow@angle\CF@default@arrow@angle\fi
	\ifx\@empty\CF@arrow@length\let\CF@arrow@length\CF@default@arrow@length\fi
	\ifx\@empty\CF@arrow@style
		\let\CF@arrow@style\CF@default@arrow@style
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\CF@arrow@style\expandafter\expandafter\expandafter
			{\expandafter\CF@default@arrow@style\expandafter,\CF@arrow@style}% se rajoute apr\`es le style par d\'efaut
	\fi
	\ifCF@reac@debug
		\tikzpicture[every node/.style={draw,anchor=base,inner sep=\z@,outer sep=\z@,minimum size=1.5pt},baseline,remember picture]%
	\else
		\tikzpicture[every node/.style={anchor=base,inner sep=\z@,outer sep=\z@,minimum size=\z@},baseline,remember picture]%
	\fi
	\let\merge\CF@merge
	\expandafter\let\csname+\endcsname\CF@and
	\let\arrow\CF@arrow
	\let\schemestop\CF@schemestop
	\let\subscheme\CF@subscheme
	\@testopt{\CF@schemestart@ii[#1]}{text}%
}

\CF@def\CF@schemestart@ii[#1][#2]{%
	\ifnum\CF@scheme@nest=\@ne% la commande n'est pas imbriqu\'ee ?
		\CF@compound@cnt\z@
	\fi
	\edef\CF@current@nodename{c\number\CF@compound@cnt}%
	\let\CF@next@nodename\@empty
	\let\CF@next@nodestyle\@empty
	\let\CF@direct@arrow@list\@empty
	\ifCF@reac@debug
		\node[fill,green](\CF@current@nodename){};%
	\else
		\node(\CF@current@nodename){};%
	\fi
	\def\CF@next@nodeanchor{#2}%
	\ifx\CF@next@nodeanchor\@empty\def\CF@next@nodeanchor{text}\fi
	\let\CF@compound\@empty
	\CF@schemestart@iii
}

\CF@def\CF@schemestart@iii{%
	\futurelet\CF@toks@a\CF@schemestart@v% va sentir le prochain token...
}

{\def\:{\CF@schemestart@iv}\expandafter}\expandafter\CF@def\: {\futurelet\CF@toks@a\CF@schemestart@v}

\CF@def\CF@schemestart@v{% ... et l'examine :
	\CF@if@firsttokin@i{\arrow\schemestop\merge}%
		\relax
		{\ifx\CF@toks@a\bgroup
			\let\CF@next@action\CF@add@nextarg
		\else
			\ifx\CF@toks@a\@sptoken
				\CF@add@tocs\CF@compound{ }%
				\let\CF@next@action\CF@schemestart@iv
			\else
				\def\CF@next@action{\CF@add@tocs\CF@compound}%
				\afterassignment\CF@schemestart@iii
			\fi
		\fi
		\CF@next@action}%
}

\CF@def\CF@add@nextarg#1{\CF@add@tocs\CF@compound{{#1}}\CF@schemestart@iii}

\CF@def\CF@display@compound#1#2{% #1 = nom et #2 = style
	\unless\ifx\@empty\CF@compound
		\global\advance\CF@compound@cnt\@ne
		\ifx\CF@default@compound@style\@empty
			\let\CF@current@nodestyle\@empty
		\else
			\expandafter\def\expandafter\CF@current@nodestyle\expandafter{\CF@default@compound@style,}%
		\fi
		\CF@add@tocs\CF@current@nodestyle{anchor=\CF@next@nodeanchor,at=(\CF@current@nodename)}%
		\ifx\@empty#2\@empty
			\unless\ifx\CF@next@nodestyle\@empty
				\CF@expadd@tocs\CF@current@nodestyle{\expandafter,\CF@next@nodestyle}%
			\fi
		\else
			\unless\ifx\CF@next@nodestyle\@empty
				\immediate\write\CF@unused{Package \CF@package@name\space Warning: two styles for the same node, first style "\CF@next@nodestyle" ignored^^J}%
			\fi
			\CF@add@tocs\CF@current@nodestyle{,#2}%
		\fi
		\ifx\@empty#1\@empty
			\edef\CF@tmp@str{\ifx\CF@next@nodename\@empty c\number\CF@compound@cnt\else\CF@next@nodename\fi}%
		\else
			\unless\ifx\CF@next@nodename\@empty
				\immediate\write\CF@unused{Package \CF@package@name\space Warning: two names for the same node, first name "\CF@next@nodename" ignored^^J}%
			\fi
			\edef\CF@tmp@str{#1}%
		\fi
		\expandafter\node\expandafter[\CF@current@nodestyle](\CF@tmp@str){\CF@compound};%
		\ifCF@reac@debug
			\node[draw=none,anchor=270,at=(\CF@tmp@str.90),fill=green!60,overlay,opacity=0.5]{\scriptsize\bfseries\CF@tmp@str};%
		\fi
		\let\CF@current@nodename\CF@tmp@str
	\fi
}

\CF@def\CF@schemestop{%
	\CF@display@compound{}{}%
	\CF@direct@arrow@list
	\endtikzpicture
	\xdef\CF@scheme@nest{\number\numexpr\CF@scheme@nest-\@ne}%
}

\CF@def\CF@analyse@arrowarg#1{\CF@analyse@arrowarg@i#1[]\@nil}

\CF@def\CF@analyse@arrowarg@i#1[#2]#3\@nil{%
	\CF@if@instr{#1}.{\CF@add@tocs\CF@tmp@str{#1[#2]}}{\CF@add@tocs\CF@tmp@str{#1.[#2]}}%
}

\CF@def\CF@arrow{%
	\@ifnextchar(%
		\CF@arrow@i
		{\@ifnextchar\bgroup{\CF@arrow@ii(.[]--.[])}{\CF@arrow@ii(.[]--.[]){}}}%
}

\CF@def\CF@arrow@i(#1--#2){%
	\def\CF@tmp@str{(}%
	\CF@analyse@arrowarg{#1}%
	\CF@add@tocs\CF@tmp@str{--}%
	\CF@analyse@arrowarg{#2}%
	\CF@add@tocs\CF@tmp@str)%
	\@ifnextchar\bgroup{\expandafter\CF@arrow@ii\CF@tmp@str}{\expandafter\CF@arrow@ii\CF@tmp@str{}}%
}

\CF@def\CF@arrow@ii(#1.#2[#3]--#4.#5[#6])#7{%
	\def\CF@current@arrowtype{#7}%
	\ifx\CF@current@arrowtype\@empty\def\CF@current@arrowtype{->}\fi
	\@testopt{\CF@arrow@iii(#1.#2[#3]--#4.#5[#6])}{}%
}

\CF@def\CF@arrow@iii(#1.#2[#3]--#4.#5[#6])[#7]{%
	\def\CF@tmp@str{\CF@arrow@v(#1.#2[#3]--#4.#5[#6])}%
	\CF@arrow@iv#7,\@empty,\@empty\@nil
}

\CF@def\CF@arrow@iv#1,#2,#3\@nil{%
	\CF@add@tocs\CF@tmp@str{{#1}}%
	\CF@expadd@tocs\CF@tmp@str{\expandafter{#2}}%
	\expandafter\CF@expadd@tocs\expandafter\CF@tmp@str\expandafter{\expandafter\expandafter\expandafter{\expandafter\CF@sanitize@lastitem#3,\@empty\@nil}}%
	\CF@tmp@str
}

% #1, #4 : nom des nodes    #2, #5 : ancres des nodes    #3, #6 : stryles des nodes
% #7 : angle fl\`eche    #8 : longueur fl\`eche    #9 : style tikz de la fl\`eche
\CF@def\CF@arrow@v(#1.#2[#3]--#4.#5[#6])#7#8#9{%
	\let\CF@arrow@current@style\CF@arrow@style
	\if\string @\expandafter\@car\detokenize{#1.}\@nil% "." au cas o\`u #1 est vide
		\if\string @\expandafter\@car\detokenize{#4.}\@nil
			\CF@expadd@tocs\CF@direct@arrow@list{\expandafter\CF@direct@arrow\expandafter{\CF@current@arrowtype}{#1}{#2}{#4}{#5}{#9}}%
			\let\CF@next@action\CF@schemestart@iii
		\else
			\unless\ifx\CF@arrow@current@style\@empty\CF@add@tocs\CF@arrow@current@style,\fi
			\ifx\@empty#9\@empty\else\CF@add@tocs\CF@arrow@current@style{#9,}\fi
			\CF@display@compound{}{#3}%
			\def\CF@next@nodename{#4}%
			\expandafter\def\expandafter\CF@current@nodename\expandafter{\@gobble#1}%
			\let\CF@arrow@start@name\CF@current@nodename
			\let\CF@arrow@end@name\CF@next@nodename
			\CF@arrow@vi{#7}{#8}{#2}{#5}%
			\def\CF@next@nodestyle{#6}%
		\fi
	\else
		\unless\ifx\CF@arrow@current@style\@empty\CF@add@tocs\CF@arrow@current@style,\fi
		\ifx\@empty#9\@empty\else\CF@add@tocs\CF@arrow@current@style{#9,}\fi
		\if\string @\expandafter\@car\detokenize{#2.}\@nil
			\errmessage{Package \CF@package@name\space Error: syntax "(<name>--@<name>)" is not allowed}%
		\else
			\CF@display@compound{#1}{#3}%
			\edef\CF@arrow@start@name{\ifx\@empty#1\@empty\CF@current@nodename\else#1\fi\ifx\@empty#2\@empty\else.#2\fi}%
			\CF@arrow@vi{#7}{#8}{#2}{#5}%
			\def\CF@next@nodename{#4}%
			\def\CF@next@nodestyle{#6}%
		\fi
	\fi
	\CF@arrow@gobspaces% mange les espaces puis ex\'ecute \CF@next@action
}

\CF@def\CF@arrow@gobspaces{\futurelet\CF@toks@a\CF@arrow@gobspaces@i}

\CF@def\CF@arrow@gobspaces@i{%
	\ifx\@sptoken\CF@toks@a
		\expandafter\CF@arrow@gobspaces@ii
	\else
		\expandafter\CF@next@action
	\fi
}

{\def\:{\CF@arrow@gobspaces@ii}\expandafter}\expandafter\def\: {\futurelet\CF@toks@a\CF@arrow@gobspaces@i}

\CF@def\CF@arrow@vi#1#2#3#4{% #1=angle   #2=longueur    #3=ancre d\'epart   #4=ancre arriv\'ee
	\def\CF@next@action{\let\CF@compound\@empty\CF@schemestart@iii}%
	\def\CF@arrow@current@angle{#1}\ifx\@empty\CF@arrow@current@angle\let\CF@arrow@current@angle\CF@arrow@angle\fi
	\def\CF@current@arrow@length{#2}\ifx\@empty\CF@current@arrow@length\let\CF@current@arrow@length\CF@arrow@length\fi
	\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@current@arrow@length*\CF@compound@sep),cyan,fill](end@arrow@i@\number\CF@scheme@nest){};%
	\edef\CF@arrow@end@name{end@arrow@i@\number\CF@scheme@nest\ifx\@empty#4\@empty\else.4\fi}%
	\ifCF@reac@debug
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@arrow@offset),red,fill](start@arrow){};%
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@current@arrow@length*\CF@compound@sep-\CF@arrow@offset),red,fill](end@arrow){};%
	\else
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@arrow@offset)](start@arrow){};%
		\node[at=(\CF@current@nodename.\ifx\@empty#3\@empty\CF@arrow@current@angle\else#3\fi),shift=(\CF@arrow@current@angle:\CF@current@arrow@length*\CF@compound@sep-\CF@arrow@offset)](end@arrow){};%
	\fi
	\def\CF@arrow@start@node{start@arrow}\def\CF@arrow@end@node{end@arrow}%
	\csname\expandafter\CF@grab@arrow@name\CF@current@arrowtype[\@nil\expandafter\expandafter\expandafter\endcsname
		\expandafter\CF@grab@arrow@args\CF@current@arrowtype[]\@nil[][][][][][][][]\@nil
	\def\CF@current@nodename{end@arrow@i@\number\CF@scheme@nest}%
	\edef\CF@next@nodeanchor{\ifx\@empty#4\@empty180+\CF@arrow@current@angle\else#4\fi}%
}

% trace un fl\`eche initi\'ee par (@nom--@nom)
% #1=type de fl\`eche   #2=nom depart   #3=ancre d\'epart    #4=nom arriv\'ee    #5=ancre arriv\'ee    #6=style fl\`eche
\CF@def\CF@direct@arrow#1#2#3#4#5#6{%
	\expandafter\def\expandafter\CF@arrow@start@name\expandafter{\@gobble#2}%
	\expandafter\def\expandafter\CF@arrow@end@name\expandafter{\@gobble#4}%
	\path[sloped,allow upside down](\@gobble#2\ifx\@empty#3\@empty\else.#3\fi)--(\@gobble#4\ifx\@empty#5\@empty\else.#5\fi)%
		coordinate[pos=0,xshift=\CF@arrow@offset](start@direct@arrow)%
		coordinate[pos=1,xshift=-\CF@arrow@offset](end@direct@arrow);%
	\def\CF@arrow@start@node{start@direct@arrow}%
	\def\CF@arrow@end@node{end@direct@arrow}%
	\pgfmathanglebetweenpoints
		{\pgfpointanchor{\@gobble#2}{\ifx\@empty#3\@empty center\else#3\fi}}
		{\pgfpointanchor{\@gobble#4}{\ifx\@empty#5\@empty center\else#5\fi}}%
	\let\CF@arrow@current@angle\pgfmathresult
	\ifx\@empty#6\@empty\else\CF@add@tocs\CF@arrow@current@style{#6,}\fi%
	\csname\CF@grab@arrow@name#1[]\@nil\expandafter\endcsname\CF@grab@arrow@args#1[]\@nil[][][][][][][][]\@nil
}

\CF@def\CF@merge@grab@chardir#1[#2][#3]#4\@nil{%
	\expandafter\futurelet\expandafter\CF@toks@a\expandafter\CF@gobble@tonil\@car#1>\@nil\@nil
	\ifx>\CF@toks@a\def\CF@merge@angle{0}\def\CF@merge@extreme{xmax}\def\CF@merge@sign{+}\else
	\ifx<\CF@toks@a\def\CF@merge@angle{180}\def\CF@merge@extreme{xmin}\def\CF@merge@sign{-}\else
	\ifx^\CF@toks@a\def\CF@merge@angle{90}\def\CF@merge@extreme{ymax}\def\CF@merge@sign{+}\else
	\ifx v\CF@toks@a\def\CF@merge@angle{-90}\def\CF@merge@extreme{ymin}\def\CF@merge@sign{-}%
	\fi\fi\fi\fi
	\def\CF@merge@labelup{#2}\def\CF@merge@labeldo{#3}%
}

\CF@def\CF@merge#1({%
	\CF@merge@grab@chardir#1[][]\@nil
	\CF@merge@i(%
}

\CF@def\CF@merge@i#1--(#2){\@testopt{\CF@merge@ii#1--(#2)}{}}

\CF@def\CF@merge@ii#1--(#2)[#3]{%
	\CF@display@compound{}{}%
	\CF@parse@mergeopt#3,\@empty,\@empty,\@empty\@nil
	\def\CF@merge@xmax{-16383.99999pt}\let\CF@merge@ymax\CF@merge@xmax
	\def\CF@merge@xmin{16383.99999pt}\let\CF@merge@ymin\CF@merge@xmin
	\CF@merge@parse@nodelist#1(\relax)% calcule les maxi des positions
	\pgfmathparse{\csname CF@merge@\CF@merge@extreme\endcsname\CF@merge@sign\CF@merge@fromcoeff*\CF@compound@sep}%
	\let\CF@merge@extreme@result\pgfmathresult
	\CF@merge@iii#1(\relax)% trace les lignes entre les noeuds pr\'ec\'edents et la ligne de jonction
	\expandafter\def\expandafter\CF@tmp@str\expandafter{\expandafter[\CF@merge@style,shorten <=0,shorten >=0]}%
	\if x\expandafter\@car\CF@merge@extreme\@nil
		\CF@add@tocs\CF@tmp@str{(\CF@merge@extreme@result pt,\CF@merge@ymax)--(\CF@merge@extreme@result pt,\CF@merge@ymin)}%
	\else
		\CF@add@tocs\CF@tmp@str{(\CF@merge@xmin,\CF@merge@extreme@result pt)--(\CF@merge@xmax,\CF@merge@extreme@result pt)}%
	\fi
	\expandafter\draw\CF@tmp@str node[pos=\CF@merge@splitcoeff](merge@point){}% trace la ligne de jonction
		node[at=(merge@point),shift=(\CF@merge@angle:\CF@compound@sep*\CF@merge@tocoeff-\CF@arrow@offset)](end@merge){}%
		node[at=(merge@point),shift=(\CF@merge@angle:\CF@compound@sep*\CF@merge@tocoeff)](end@merge@i){};%
	\let\CF@arrow@current@angle\CF@merge@angle
	\expandafter\draw\expandafter[\CF@merge@style,shorten <=0,-CF@full](merge@point)--(end@merge)%
		\expandafter\CF@arrow@display@label@i\expandafter{\CF@merge@labelup}{.5}+\expandafter\CF@arrow@display@label@i\expandafter{\CF@merge@labeldo}{.5}-;%
	\def\CF@current@nodename{end@merge@i}%
	\let\CF@tmp@str\@empty
	\CF@analyse@arrowarg{#2}%
	\expandafter\CF@merge@iv\CF@tmp@str\@nil
}

\CF@def\CF@merge@iii(#1){%
	\if\relax\expandafter\noexpand\@car#1\@nil
	\else
		\CF@if@stop{#1}%
			{\edef\merge@current@nodename{\CF@before@stop#1\@nil}\edef\merge@current@anchor{\CF@after@stop#1\@nil}}%
			{\def\merge@current@nodename{#1}\let\merge@current@anchor\CF@merge@angle}%
		\if x\expandafter\@car\CF@merge@extreme\@nil
			\pgfextracty\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
			\expandafter\draw\expandafter[\CF@merge@style,shorten >=0]([shift=(\CF@merge@angle:\CF@arrow@offset)]\merge@current@nodename.\merge@current@anchor)--(\CF@merge@extreme@result pt,\CF@dim);%
		\else
			\pgfextractx\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
			\expandafter\draw\expandafter[\CF@merge@style,shorten >=0]([shift=(\CF@merge@angle:\CF@arrow@offset)]\merge@current@nodename.\merge@current@anchor)--(\CF@dim,\CF@merge@extreme@result pt);%
		\fi
		\expandafter\CF@merge@iii
	\fi
}

\CF@def\CF@merge@iv#1.#2[#3]\@nil{%
	\def\CF@next@nodename{#1}%
	\edef\CF@next@nodeanchor{\ifx\@empty#2\@empty180+\CF@merge@angle\else#2\fi}%
	\def\CF@next@nodestyle{#3}%
	\let\CF@compound\@empty
	\CF@schemestart@iii
}

\CF@def\CF@parse@mergeopt#1,#2,#3,#4\@nil{%
	\def\CF@merge@fromcoeff{#1}\ifx\@empty\CF@merge@fromcoeff\def\CF@merge@fromcoeff{0.5}\fi
	\expandafter\def\expandafter\CF@merge@tocoeff\expandafter{#2}\ifx\@empty\CF@merge@tocoeff\def\CF@merge@tocoeff{0.5}\fi
	\expandafter\def\expandafter\CF@merge@splitcoeff\expandafter{#3}\ifx\@empty\CF@merge@splitcoeff\def\CF@merge@splitcoeff{0.5}\fi
	\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\CF@merge@style\expandafter\expandafter\expandafter{\expandafter\CF@sanitize@lastitem#4,\@empty\@nil}%
}

\CF@def\CF@merge@parse@nodelist(#1){%
	\if\relax\expandafter\noexpand\@car#1\@nil
	\else
		\CF@if@stop{#1}%
			{\edef\merge@current@nodename{\CF@before@stop#1\@nil}\edef\merge@current@anchor{\CF@after@stop#1\@nil}}%
			{\def\merge@current@nodename{#1}\let\merge@current@anchor\CF@merge@angle}%
		\pgfextractx\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
		\ifdim\CF@dim>\CF@merge@xmax\edef\CF@merge@xmax{\the\CF@dim}\fi
		\ifdim\CF@dim<\CF@merge@xmin\edef\CF@merge@xmin{\the\CF@dim}\fi
		\pgfextracty\CF@dim{\pgfpointanchor\merge@current@nodename\merge@current@anchor}%
		\ifdim\CF@dim>\CF@merge@ymax\edef\CF@merge@ymax{\the\CF@dim}\fi
		\ifdim\CF@dim<\CF@merge@ymin\edef\CF@merge@ymin{\the\CF@dim}\fi
		\expandafter\CF@merge@parse@nodelist
	\fi
}

\CF@def\CF@grab@arrow@name#1[#2\@nil{#1}
\CF@def\CF@grab@arrow@args#1[#2\@nil{[#2}

\CF@def\CF@make@parameter@text#1{%
	\toks\z@{}%
	\CF@cnt@groupnumber#1\relax
	\CF@make@parameter@text@i1%
}

\CF@def\CF@make@parameter@text@i#1{%
	\unless\ifnum#1>\CF@cnt@groupnumber
		\toks\z@\expandafter{\the\toks\z@[###1]}%
		\expandafter\CF@make@parameter@text@i\expandafter{\number\numexpr#1+1\expandafter}%
	\fi
}

% #1 est le nombre d'arguments optionnels, #2 est le nom et #3 le code
\CF@def\definearrow#1#2#3{%
	\begingroup
		\CF@make@parameter@text{#1}%
	\expandafter\endgroup
	\expandafter\def\csname\detokenize{#2}\expandafter\endcsname\the\toks\z@{#3\CF@gobble@tonil}%
}

\CF@def\CF@if@stop#1{\CF@if@stop@i#1.\@nil}
\CF@def\CF@if@stop@i#1.#2\@nil{\ifx\@empty#2\@empty\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}
\CF@def\CF@before@stop#1.#2\@nil{#1}
\CF@def\CF@after@stop#1.#2\@nil{#2}

\CF@def\CF@rotate@node*#1#2\@nil{\CF@if@stop{#1}{\CF@before@stop#1\@nil}{#1}}
\CF@def\CF@anchor@node*#1#2\@nil#3{\CF@if@stop{#1}{\CF@after@stop#1\@nil}{\CF@arrow@current@angle-#390-#1}}

% #1 = label  #2 = position  #3 = + ou - (au dessus ou au dessous)  #4 : nom du noeud de d\'epart
% #5 = label  #6 = position  #7 = + ou - (au dessus ou au dessous)  #8 : nom du noeud de fin
\CF@def\CF@arrow@display@label#1#2#3#4#5#6#7#8{%
	\ifx\@empty#1#5\@empty\else
		\path(#4)--(#8)\CF@arrow@display@label@i{#1}{#2}{#3}\CF@arrow@display@label@i{#5}{#6}{#7};%
	\fi
}

\CF@def\CF@arrow@display@label@i#1#2#3{%
	\ifx\@empty#1\@empty\else
		\if*\expandafter\@car\detokenize{#1}\@nil
			\ifCF@reac@debug
				node[pos=#2,sloped,yshift=#3\CF@arrow@labelsep,draw,fill,cyan](shifted@node){}%
				node[draw,rotate=\CF@rotate@node#1\@nil,anchor=\CF@anchor@node#1\@nil#3,at=(shifted@node)]{\expandafter\@gobble\@gobble#1}%
			\else
				node[pos=#2,sloped,yshift=#3\CF@arrow@labelsep](shifted@node){}%
				node[rotate=\CF@rotate@node#1\@nil,anchor=\CF@anchor@node#1\@nil#3,at=(shifted@node)]{\expandafter\@gobble\@gobble#1}%
			\fi
		\else
			\ifCF@reac@debug
				node[pos=#2,sloped,yshift=#3\CF@arrow@labelsep,draw,fill,cyan](shifted@node){}%
				node[draw,pos=#2,anchor=-#390,sloped,yshift=#3\CF@arrow@labelsep]{#1}%
			\else
				node[pos=#2,anchor=-#390,sloped,yshift=#3\CF@arrow@labelsep]{#1}%
			\fi
		\fi
	\fi
}

% pose des noeuds d\'ecal\'es de la dimension #1 \`a (\CF@arrow@start@node) et (\CF@arrow@end@node)
\CF@def\CF@arrow@shift@nodes#1{%
	\unless\ifdim\ifx\@empty#1\@empty\z@\else#1\fi=\z@
		\edef\CF@tmp@str{%
			\noexpand\path(\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0,sloped,yshift=#1](\CF@arrow@start@node1){}node[pos=1,sloped,yshift=#1](\CF@arrow@end@node1){};}%
		\CF@tmp@str
		\edef\CF@arrow@start@node{\CF@arrow@start@node1}\edef\CF@arrow@end@node{\CF@arrow@end@node1}%
	\fi
}

\definearrow3{->}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow3{<-}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@full-](\CF@arrow@start@node)--(\CF@arrow@end@node);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow5{-/>}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node)%
		coordinate[midway,shift=(\CF@arrow@current@angle:-1pt)](midway@i)%
		coordinate[midway,shift=(\CF@arrow@current@angle:1pt)](midway@ii)%
		coordinate[at=(midway@i),shift=(\ifx\@empty#4\@empty225\else#4+180\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@start)%
		coordinate[at=(midway@i),shift=(\ifx\@empty#4\@empty45\else#4\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@end)%
		coordinate[at=(midway@ii),shift=(\ifx\@empty#4\@empty225\else#4+180\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@start@i)%
		coordinate[at=(midway@ii),shift=(\ifx\@empty#4\@empty45\else#4\fi+\CF@arrow@current@angle:\ifx\@empty#5\@empty5pt\else#5\fi)](line@end@i);
	\draw(line@start)--(line@end);%
	\draw(line@start@i)--(line@end@i);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow3{<->}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@full-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow3{<=>}{%
	\CF@arrow@shift@nodes{#3}%
	\edef\CF@tmp@str{%
		\noexpand\path[allow upside down](\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0,sloped,yshift=1pt](\CF@arrow@start@node @u0){}%
			node[pos=0,sloped,yshift=-1pt](\CF@arrow@start@node @d0){}%
			node[pos=1,sloped,yshift=1pt](\CF@arrow@start@node @u1){}%
			node[pos=1,sloped,yshift=-1pt](\CF@arrow@start@node @d1){};%
		}%
	\CF@tmp@str
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@half](\CF@arrow@start@node @u0)--(\CF@arrow@start@node @u1);%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@half-](\CF@arrow@start@node @d0)--(\CF@arrow@start@node @d1);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node%
}

\definearrow3{<->>}{%
	\CF@arrow@shift@nodes{#3}%
	\edef\CF@tmp@str{%
		\noexpand\path[allow upside down](\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0,sloped,yshift=1pt](\CF@arrow@start@node @u0){}%
			node[pos=0.2,sloped,yshift=-1pt](\CF@arrow@start@node @d0){}%
			node[pos=1,sloped,yshift=1pt](\CF@arrow@start@node @u1){}%
			node[pos=0.8,sloped,yshift=-1pt](\CF@arrow@start@node @d1){};%
		}%
	\CF@tmp@str
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@half](\CF@arrow@start@node @u0)--(\CF@arrow@start@node @u1);%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@half-](\CF@arrow@start@node @d0)--(\CF@arrow@start@node @d1);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node%
}

\definearrow3{<<->}{%
	\edef\CF@tmp@str{%
		\noexpand\path[allow upside down](\CF@arrow@start@node)--(\CF@arrow@end@node)%
			node[pos=0.2,sloped,yshift=1pt](\CF@arrow@start@node @u0){}%
			node[pos=0,sloped,yshift=-1pt](\CF@arrow@start@node @d0){}%
			node[pos=0.8,sloped,yshift=1pt](\CF@arrow@start@node @u1){}%
			node[pos=1,sloped,yshift=-1pt](\CF@arrow@start@node @d1){};%
		}%
	\CF@tmp@str
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@half](\CF@arrow@start@node @u0)--(\CF@arrow@start@node @u1);%
	\expandafter\draw\expandafter[\CF@arrow@current@style,CF@half-](\CF@arrow@start@node @d0)--(\CF@arrow@start@node @d1);%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node
}

\definearrow30{%
	\CF@arrow@shift@nodes{#3}%
	\CF@arrow@display@label{#1}{0.5}+\CF@arrow@start@node{#2}{0.5}-\CF@arrow@end@node}

\definearrow5{-U>}{%
	\CF@arrow@shift@nodes{#3}%
	\expandafter\draw\expandafter[\CF@arrow@current@style,-CF@full](\CF@arrow@start@node)--(\CF@arrow@end@node)node[midway](Uarrow@arctangent){};%
	\edef\CF@tmp@str{[\ifx\@empty#1\@empty draw=none\else\unexpanded\expandafter{\CF@arrow@current@style}\fi]}%
	\expandafter\draw\CF@tmp@str (Uarrow@arctangent)%
		arc[radius=\CF@compound@sep*\CF@current@arrow@length*\ifx\@empty#4\@empty0.333\else#4\fi,start angle=\CF@arrow@current@angle-90,%
		delta angle=-\ifx\@empty#5\@empty60\else#5\fi]node(Uarrow@start){};
	\edef\CF@tmp@str{[\ifx\@empty#2\@empty draw=none\else\unexpanded\expandafter{\CF@arrow@current@style},-CF@full\fi]}%
	\expandafter\draw\CF@tmp@str (Uarrow@arctangent)%
		arc[radius=\CF@compound@sep*\CF@current@arrow@length*\ifx\@empty#4\@empty0.333\else#4\fi,start angle=\CF@arrow@current@angle-90,%
		delta angle=\ifx\@empty#5\@empty60\else#5\fi]node(Uarrow@end){};
	\pgfmathparse{#51*#41*cos(\CF@arrow@current@angle)<0?"-":"+"}\let\CF@tmp@str\pgfmathresult
	\CF@arrow@display@label{#1}{0}\CF@tmp@str{Uarrow@start}{#2}{1}\CF@tmp@str{Uarrow@end}%
}

\pgfarrowsdeclare{CF@half}{CF@half}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfarrowsleftextend{-\CF@arrow@size}\pgfarrowsrightextend{.5\pgflinewidth}}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfsetdash{}\z@\pgfsetroundjoin\pgfsetroundcap
	\pgfpathmoveto{\pgfpoint\z@\z@}%
	\pgfpathlineto{\pgfpoint{-\CF@arrow@size}{.5\CF@arrow@size}}%
	\pgfpathlineto{\pgfpoint{-.5\CF@arrow@size}\z@}%
	\pgfpathlineto{\pgfpoint\z@\z@}%
	\pgfusepathqfillstroke}

\pgfarrowsdeclare{CF@full}{CF@full}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfarrowsleftextend{-\CF@arrow@size}\pgfarrowsrightextend{.5\pgflinewidth}}%
	{\CF@arrow@size\dimexpr2.5pt+2.5\pgflinewidth\relax
	\pgfsetdash{}\z@\pgfsetroundjoin\pgfsetroundcap
	\pgfpathmoveto{\pgfpoint\z@\z@}%
	\pgfpathlineto{\pgfpoint{-\CF@arrow@size}{.5\CF@arrow@size}}%
	\pgfpathlineto{\pgfpoint{-.5\CF@arrow@size}\z@}%
	\pgfpathlineto{\pgfpoint{-\CF@arrow@size}{-.5\CF@arrow@size}}%
	\pgfpathlineto{\pgfpoint\z@\z@}%
	\pgfusepathqfillstroke}

\chemfigrestorecatcode

\endinput

######################################################################
#                             Historique                             #
######################################################################

v0.1        2010/06/23
    - Premi\`ere version publique sur le CTAN
----------------------------------------------------------------------
v0.2        2010/08/31
    - Ajout de la documentation en anglais.
    - Correction de bugs.
    - \printatom est d\'esormais une macro publique.
    - Les espaces sont permis dans les mol\'ecules. Ils seront
      ignor\'es par d\'efaut puisque les atomes sont compos\'es en
      mode math par \printatom
    - Une paire de Lewis peut \^etre repr\'esent\'ee ":".
    - Dans les cycles, une correction de la longueur du trait
      d\'eport\'e des liaisons doubles est fait de telle sorte que si
      l'on \'ecrit \chemfig{*5(=====)}, on obtient deux polygones
      r\'eguliers concentriques.
    - La s\'equence de contr\^ole \setnodestyle permet de sp\'ecifier
      le style des noeuds dessin\'es par tikz.
----------------------------------------------------------------------
v0.3        2010/11/21
    - Am\'elioration de \definesubmol qui accepte les s\'equences de
      contr\^ole. On peut aussi choisir un alias dont la substitution
      est diff\'erente selon l'orientation de la liaison qui lui
      arrive dessus.
    - Le caract\`ere "|" force la fin d'un atome. Si on \'ecrit
      "D|ef" alors, chemfig verra deux atomes "D" et "ef".
    - Le caract\`ere "#" est reconnu lorsqu'il suit un caract\`ere de
      liaison. Il doit \^etre suivi d'un argument entre parenth\`eses
      qui contient l'offset de d\'ebut et de fin qui s'appliqueront
      \`a cette liaison.
    - La macro \chemfig admet un argument optionnel qui sera pass\'e
      \`a l'environnement tikzpicture dans lequel elle est dessin\'ee
    - Mise en place de la repr\'esentation des m\'ecanismes
      r\'eactionnels avec la synatxe "@{<nom>}" devant un atome o\`u
      "@{<nom>,<coeff>}" au tout d\'ebut de l'argument d'une liaison.
      Cette syntaxe permet de placer un noeud (au sens de tikz) qui
      deviendra l'extr\'emit\'e des fl\`eches des m\'ecanismes.
      Le trac\'e des fl\`eches est faite par la macro \chemmove dont
      l'argument optionnel devient celui de l'environnement
      tikspicture dans lequel sont faites les fl\`eches.
    - Pour le m\'ecanisme d'alignement vertical via le \vphantom, la
      commande \chemskipalign permet d'ignorer le groupe d'atomes
      dans lequel elle est \'ecrite.
    - La commande \chemname permet d'afficher un nom sous une
      mol\'ecule. la commande \chemnameinit initialise la plus grande
      profondeur rencontr\'ee.
    - La commande \lewis a \'et\'e modifi\'ee de telle sorte que les
      dessins des d\'ecorations soient proportionnels \`a la taille
      de la police.
----------------------------------------------------------------------
v0.3a       2011/01/08
    - Correction d'un bug dans l'argument optionnel de \definesubmol
      lorsque celui-ci comporte des crochets.
    - Mise \`a jour du manuel en anglais.
    - Ajout de \vflipnext et \hflipnext pour retourner
      horizontalement ou verticalement la prochaine mol\'ecule.
----------------------------------------------------------------------
v0.4        2011/03/07
    - chemfig est d\'esormais \'ecrit en plain-etex et donc
      utilisable par d'autres formats que LaTeX.
    - Un peu plus de rigueur avec les catcodes des caract\`eres
      sp\'eciaux, notamment lorsque la commande \chemfig se trouve
      dans l'argument de \chemmove, \chemabove, \chembelow, \chemrel.
      TODO : faut-il \scantoker l'argument de \chemfig pour \^etre
      d\'efinitivement d\'ebarass\'e de ces histoires de catcode ???
    - Correction d'un bug dans le calcul de l'angle des liaisons
----------------------------------------------------------------------
v0.4a       2011/04/10
    - Correction d'un bug concernant l'argument optionnel en d\'ebut
      de mol\'ecule.
----------------------------------------------------------------------
v0.4b       2011/04/24
    - l'argument de \chemfig est tok\'enis\'e avec \scantokens ce qui
      rend caduc tout souci de code de cat\'egorie, \`a part #.
    - la commande \setbondstyle permet de d\'efinir le style des
      liaisons.
    - correction de l'affichage incorrect des doubles liaisons dans
      les cycles apr\`es les commandes \hflipnext et \vflipnext
    - correction d'un bug lorsqu'un alias commence une mol\'ecule
----------------------------------------------------------------------
v1.0       2011/06/15
    - les sch\'emas r\'eactionnels sont d\'esormais disponibles.
    - \Chemabove et \Chembelow modifient la boite englobante.
    - \Lewis modifie la boite englobante
    - les macros \chemleft, \chemright, \chemup et \chemdown
      affichent des d\'elimiteurs extensibles \`a gauche, \`a droite,
      au dessus et au dessous d'un mat\'eriel.
----------------------------------------------------------------------
v1.0a      2011/09/18
    - les macros \Lewis et \lewis admettent un argument optionnel
    - la macro \setlewisdist r\`egle la distance entre les 2
      \'electrons
----------------------------------------------------------------------
v1.0b      2011/11/29
    - la commande \merge est d\'esormais prot\'eg\'ee entre
      \schemestart et \schemestop contre des d\'efinitions par d'autres
      packages.
    - \box\z@ est utilis\'e au lieu du maladroit \unhbox\z@
----------------------------------------------------------------------
v1.0c      2011/11/30
    - la macro \+ n'est plus explicitement \'ecrite
    - v\'erifie que eTeX est le moteur utilis\'e
----------------------------------------------------------------------
v1.0d      2011/12/19
    - les cercles des cycles \'etaient trac\'es au mauvais moment. La
      longueur de la liaison qui les pr\'ec\'edait influait sur le
      rayon du cercle : \chemfig{-[,0.5]**6(------)} donnait un bug
      \`a l'affichage.
----------------------------------------------------------------------
v1.0e      2012/01/13
    - la gestion des espaces dans les groupes d'atomes est
      d\'esormais plus rigoureuse. Plusieurs bugs ont \'et\'e
      corrig\'e
----------------------------------------------------------------------
v1.0f      2012/02/24
    - correction d'un bug avec \definesubmol, les catcodes n'\'etaient
      pas correctement g\'er\'es.
----------------------------------------------------------------------
v1.0g      2012/11/16
    - correction d'un bug dans \CF@direct@arrow pour faire prendre en
      compte le style des fl\`eche par d\'efaut
    - correction d'un bug dans \CF@lewis@iii : la boite *doit* \^etre
      compos\'ee en dehors de l'environnement tikzpicture pour
      \'eviter nullfont si jamais \printatom ne passe pas en mode
      math.
    - correction d'un bug dans \CF@chemfig@v : si une longueur par
      d\'efaut est modifi\'ee par [,<l>] au d\'ebut d'une mol\'ecule
      et si des cycles \'etaient emboit\'es, cette longueur n'\'etait
      pas appliqu\'ee aux sous-cycles.
    - r\'e-\'ecriture des macros \chemabove et \chembemow pour
      prendre en compte le bug (d\'esormais corrig\'e) dans luatex.
    - nouvelle macro \setstacksep qui d\'efinit l'espacement par
      d\'efaut dans les macros \chemabove et \chembelow.
----------------------------------------------------------------------
v1.0h      2013/11/28
    - \chemname admet maintenant une version \'etoil\'e qui ne tient
      pas compte des profondeurs pr\'ec\'edentes.
    - \CF@dp@max est g\'er\'e globalement.
    - correction d'un bug dans "-U>" : le style de la fl\`eche
      n'\'etait pris en compte pour l'arc.
    - correction d'un bug dans \CF@direct@arrow : l'angle de la
      fl\`eche n'\'etait pas calcul\'e
----------------------------------------------------------------------
v1.1       2015/02/13
    - correction d'un bug dans \CF@seek@submol : la macro
      \CF@remain@molecule est d\'epouill\'e de son \'eventuel espace
      en premi\`ere position.
    - correction d'un bug dans \CF@arrow@vi : le nom du prochain
      noeud courant "end@arrow@i" \'etait erron\'e dans le cas o\`u une
      fl\`eche contenait un sous sch\'ema. Ce nom doit d\'ependre de
      \CF@scheme@nest.
    - la jonction entre deux liaisons cons\'ecutives dans l'axe peut
      \^etre activ\'e avec \enablebondjoin et d\'esactiv\'e avec
      \disablebondjoin (pr\'ef\'erable, \'etat par d\'efaut).
    - \chemfig suivi d'une "*" demande \`a ce que les liaisons aient
      une longueur invariable : la distance inter-atome devient donc
      variable. Cette fonctionnalit\'e est d\'esavctiv\'e dans les
      cycles afin que les polygones soient r\'eguliers.
      \enablefixedbondlength permet cette fonctionnalit\'e pour
      toutes les macros \chemfig (m\^eme non \'etoil\'ee) tandis que
      \disablefixedbondlength le d\'esactive.
----------------------------------------------------------------------
v1.1a      2015/02/23
    - correction d'un bug dans \CF@grab@bondoffset. Si \chemfig est
      dans l'argument d'une macro, les # sont doubl\'es par l'action
      de \scantokens de la macro \CF@chemfig@iv et il faut un
      argument d\'elimit\'e avant "(" pour absorber tous les #.
